$AdS_5\times S^5$ mirror TBA equations from Y-system and discontinuity relations

Using the recently proposed set of discontinuity relations we translate the AdS/CFT Y-system to TBA integral equations and quantization conditions for a large subset of excited states from the sl(2) sector of the $AdS_5 \times S^5$ string sigma-model. Our derivation provides an analytic proof of the fact that the exact Bethe equations reduce to the Beisert-Staudacher equations in the asymptotic limit. We also construct the corresponding T-system and show that in the language of T-functions the energy formula reduces to a single term which depends on a single T-function.

==> nlie2 <==
%\cite{Hegedus:2006st}
%\bibitem{Hegedus:2006st}
  A.~Hegedus, F.~Ravanini and J.~Suzuki,
 %``Exact finite size spectrum in super sine-Gordon model,''
  Nucl.\ Phys.\  B {\bf 763} (2007) 330
  [arXiv:hep-th/0610012].
  %%CITATION = NUPHA,B763,330;%%
%\cite{Dunning:2002tt}
%\bibitem{Dunning:2002tt}
  C.~Dunning,
 %``Finite size effects and the supersymmetric sine-Gordon models,''
  J.\ Phys.\ A  {\bf 36} (2003) 5463
  [arXiv:hep-th/0210225].
  %%CITATION = JPAGB,A36,5463;%%
%\cite{Hegedus:2003xd}
%\bibitem{Hegedus:2003xd}
  A.~Hegedus,
 %``Finite size effects in the SS model: Two component nonlinear integral
  %equations,''
  Nucl.\ Phys.\  B {\bf 679} (2004) 545
  [arXiv:hep-th/0310051].
  %%CITATION = NUPHA,B679,545;%%
%\cite{Hegedus:2004xd}
%\bibitem{Hegedus:2004xd}
  A.~Hegedus,
 ``Nonlinear integral equations for finite volume excited state energies of
  %the O(3) and O(4) nonlinear sigma-models,''
  J.\ Phys.\ A  {\bf 38} (2005) 5345
  [arXiv:hep-th/0412125].
  %%CITATION = JPAGB,A38,5345;%%
%\cite{Gromov:2008gj}
%\bibitem{Gromov:2008gj}
  N.~Gromov, V.~Kazakov and P.~Vieira,
 %``Finite Volume Spectrum of 2D Field Theories from Hirota Dynamics,''
  JHEP {\bf 0912} (2009) 060
  [arXiv:0812.5091 []].
  %%CITATION = JHEPA,0912,060;%%
%\cite{Balog:2009ze}
%\bibitem{Balog:2009ze}
  J.~Balog and A.~Hegedus,
 %``The finite size spectrum of the 2-dimensional O(3) nonlinear sigma-model,''
  Nucl.\ Phys.\  B {\bf 829} (2010) 425
  [arXiv:0907.1759 []].
%%CITATION = NUPHA,B829,425;%%


==> nzQC <==
In this section we formulate the quantization conditions and the exact
Bethe equations which determine the discreet parameters $\xi_{m,j}$,
$\tilde\xi_{m,j}$ and $u_j$ occurring in the source terms of the TBA
integral equations. 

\subsection{Quantization conditions}

In this subsection we quantize the roots occurring in the functions
\begin{equation}
\tau_m(u)=\prod_{j=1}^{{\cal N}_m}t(u-\xi_{m,j}),\qquad
\tilde\tau_m(u)=\prod_{j=1}^{\tilde{\cal N}_m}t(u-\tilde\xi_{m,j}),\qquad
m=2,3,\dots
\end{equation}
(Note that $\tilde\tau_1(u)\equiv1$ and the physical rapidities $u_j$
occurring in $\tau_1(u)=\prod t(u-u_j)$ will be quantized by the exact Bethe
equations discussed in the next subsection.)
We assume that (as is the case in the asymptotic solution) the
functions $Y_{m\vert vw}^{[\pm2]}$ have no poles around the points $\xi_{m,j}$
or $\xi_{m+2,j}$ and therefore the zeroes on the left hand side of the
Y-system equations (\ref{Ymvw}) must be accompanied by corresponding
zeroes also on the right hand side. This leads to the quantization
conditions
\begin{equation}
1+Y^\pm_{m\vert vw}(\xi_{m+1,j})=0,\qquad m=1,2,\dots,\qquad
j=1,\dots,{\cal N}_{m+1}.
\end{equation}
These are well-defined even for $m=1$ since
\begin{equation}
\frac{Y_{1\vert vw}^+(\xi_{2,j}+i\epsilon)}
{Y_{1\vert vw}^+(\xi_{2,j}-i\epsilon)}=
\frac{1-Y_-(\xi_{2,j}+i\epsilon)}
{1-Y_+(\xi_{2,j}+i\epsilon)}=1.
\end{equation}

Similarly we assume that the functions $Y_{m\vert w}^{[\pm2]}$ have no 
poles around the points $\tilde\xi_{m,j}$ or $\tilde\xi_{m+2,j}$ and 
therefore we have the quantization conditions
\begin{equation}
1+Y^\pm_{m\vert w}(\tilde\xi_{m+1,j})=0,\qquad m=1,2,\dots,\qquad
j=1,\dots,\tilde{\cal N}_{m+1}.
\end{equation}
These are well-defined even for $m=1$.

We discuss an important special case in detail. In this special case
(which is relevant for example for the case of twist-two states in the
${\alg{sl}(2)}$ sector) we have no $\tilde\xi_{m,j}$ rootes at all and all
$\xi_{m,j}$ roots are real. Moreover all ${\cal N}_m$ are even numbers.
Then we can make the following definitions. The (\ref{TBAmvw}-\ref{TBA1vw})
TBA equations can be written
\begin{equation}
Y_{m\vert vw}=\tau_m\tau_{m+2}\exp\left\{f_m\star s\right\},
\end{equation}
where
\begin{equation}
f_m(u)=\ln\left(\frac{[1+Y_{m-1\vert vw}(u)][1+Y_{m+1\vert vw}(u)]}
{1+Y_{m+1}(u)}\right)+\Theta(4-u^2)\delta_{m,1}\ln\left(\frac{
1-Y_-(u)}{1-Y_+(u)}\right)
\end{equation}
and we define
\begin{equation}
{\cal B}_m(u)=\frac{g}{4}\,{\cal P}\,\int_{-\infty}^\infty{\rm d}v\,
\frac{f_m(v)}{\sinh\frac{(u-v)g\pi}{2}}.
\end{equation}
Note that the principal value prescription ${\cal P}$ is actually
superfluous at the points we will need this function since
\begin{equation}
f_m(\xi_{m+1,j})=0,\qquad m=1,2,\dots,\qquad j=1,\dots,{\cal N}_{m+1}.
\end{equation}
We also define
\begin{equation}
R_m(u)=2\sum_{j=1}^{{\cal N}_m}\arctan\tanh\frac{(u-\xi_{m,j})g\pi}{4}.
\end{equation}
In the special case the quantization conditions take the form 
\begin{equation}
R_m(\xi_{m+1,k})+R_{m+2}(\xi_{m+1,k})+{\cal B}_m(\xi_{m+1,k})=
2\pi\nu_{m+1,k}\quad m=1,2,\dots,\quad k=1,\dots,{\cal N}_{m+1},
\end{equation}
where
\begin{equation}
\nu_{m+1,k}=\left\{
\begin{split}
{\rm integer\ \ \ \ \ \ } \quad {\rm if}\quad
 &\frac{{\cal N}_m+{\cal N}_{m+2}}{2} \quad {\rm is\ odd},\\
{\rm half-integer} \qquad {\rm if} \quad 
&\frac{{\cal N}_m+{\cal N}_{m+2}}{2} \quad {\rm is\ even}.
\end{split}
\right.
\end{equation}

\subsection{Exact Bethe equations}

The quantization conditions for the physical rapidities $u_k$ are
the exact Bethe equations:
\begin{equation}
Y_{1(*)}(u_k)=-1,\qquad   k=1,2,\dots,N,
\end{equation}
where the analytic continuation (denoted by the subscript $_{(*)}$) means that
we have to analytically continue the function from the real line just below the
cut line at $-\frac{i}{g}$ coming down between the branch points 
$\pm2-\frac{i}{g}$, and then going back to the real axis through the cut.
Using our previously introduced notation, for the function $F(u)$ we have
\begin{equation}
F_{(*)}(u)=\left(\left(F^-\right)_*\right)^+(u-i\epsilon).
\end{equation}
Our definition is in agreement with the transformation rules
$x^\pm_{(*)}(u)=x^\pm_s(u)$ and \hfill\break
$S^{1*\,1}_{{\alg{sl}(2)}(*)}(u_j,u)=S^{1*\,1*}_{{\alg{sl}(2)}}(u_j,u)$.
It is also easy to see that the following transformation rules hold:
\begin{eqnarray}
f=F\ \check\star\ K_1  
\quad\Rightarrow\quad f_{(*)}(u)&=&f(u)-F^+(u-i\epsilon),\\
\psi=F\ \hat\star\  K_1\quad\Rightarrow\quad 
\psi_{(*)}(u)&=&\psi(u)+F_*^+(u-i\epsilon).
\end{eqnarray}
Using the last formula we can write the following further identities
\begin{eqnarray}
\left(F\ \hat\star\ K^{y1}_+\right)_{(*)}&=&F\ \hat\star\ K^{y1}_{+(*)},\\
\left(F\ \hat\star\ K^{y1}_-\right)_{(*)}&=&F\ \hat\star\ K^{y1}_{-(*)}
+F^{[1-\epsilon]}_*,\\
\left(F\ \hat\star\ K_{y1}\right)_{(*)}&=&F\ \hat\star\ K_{y1(*)}
+F^{[1-\epsilon]}_*.
\end{eqnarray}

Using this set of identities we can rewrite the exact Bethe equations:
\begin{equation}
\ln Y_{1(*)}(u_k)=2\pi i\nu_k,\qquad \nu_k:{\rm \ half-integer},\qquad
k=1,\dots,N, 
\end{equation}
where
\begin{equation}
\begin{split}
\ln Y_{1(*)}=&-L\ln(x^+x^-)+f_{1(*)}+2r_1\star s^{[\epsilon-1]}+
2r_1\star s\ \hat\star\ K_{y1(*)}\\
&-2\ln\left[\frac{1-Y_-}{1-Y_+}\right]\ \hat\star\ s\star K^{11}_{vwx(*)}
+2{\mathscr L}_-\ \hat\star\ K^{y1}_{-(*)}
+2{\mathscr L}_+\ \hat\star\ K^{y1}_{+(*)}\\
&+2{\mathscr L}_+^{[1-\epsilon]}+\sum_{Q=1}^\infty L_Q\star\left\{
K^{Q1}_{{\alg{sl}(2)}(*)}+2s\star K^{Q-1\,1}_{vwx(*)}\right\}
\end{split}
\label{BY}
\end{equation}
and
\begin{equation}
f_{1(*)}(u)=-\sum_{j=1}^N\ln S^{1*\,1*}_{{\alg{sl}(2)}}(u_j,u)-2\left(T^{[\epsilon]}
\star K^{11[\epsilon]}_{vwx(*)}\right)(u).
\label{f1star}
\end{equation}
We note that since
\begin{equation}
2{\mathscr L}_+^+=-2iR_2+\ln\left(1-\frac{1}{Y_+^+}\right)^2
\end{equation}
and here the second term vanishes at $u_k$, the first term in the third
line in (\ref{BY}) can be substituted by $-2iR_2$. We also note that the
$\epsilon$ prescription in the third term in (\ref{BY}) is not really needed
since $r_1$ vanishes at $u=u_k$.

Finally we give an alternative variant of (\ref{f1star}) using the 
regularization introduced in~\cite{Arutyunov:2009ax}:
\begin{equation}
\begin{split}
f_{1(*)}(u)=&-\sum_{j=1}^N\ln S^{1*\,1*}_{{\alg{sl}(2)}}(u_j,u)+
2\int_{-\infty}^\infty{\rm d}v\,\ln\frac{Q(v)}{\tau_1(v)}\,K^{11}_{vwx(*)}
(v+i\epsilon,u)\\
&-2\sum_{j=1}^N\ln\left[(u_j-u^{++})\,\frac{x_j^--\frac{1}{x^-(u)}}
{x_j^--x^+(u)}\right].
\end{split}
\end{equation}
At $u=u_k$, where we need it, we have
\begin{equation}
\begin{split}
f_{1(*)}(u_k)=&-\sum_{j=1}^N\ln S^{1*\,1*}_{{\alg{sl}(2)}}(u_j,u_k)+
2\int_{-\infty}^\infty{\rm d}v\,\ln\frac{Q(v)}{\tau_1(v)}\,K^{11}_{vwx(*)}
(v+i\epsilon,u_k)\\
&-2\sum_{j=1}^N\ln\left[(u_j-u_k-\frac{2i}{g})\,\frac{x_j^--\frac{1}{x_k^-}}
{x_j^--\frac{1}{x_k^+}}\right].
\end{split}
\end{equation}

Again, the final formula for the exact Bethe-Yang equations agrees with
the results obtained in \cite{Arutyunov:2009ax} by contour deformation 
techniques.


==> nzappC <==


\subsection{Asymptotic transfer matrices}

In the asymptotic limit the $Y_{Q,0}$ functions tend to zero and the Y-system of AdS/CFT splits into
two $SU(2|2)$ Y-systems. Correspondingly two independent $SU(2|2)$ T-systems generates the asymptotic
solutions for the Y-functions. The asymptotic solution being consisitent with the asymptotic Bethe Ansatz
equations \cite{BS} and the multiparticle L\"uscher formulae \cite{BJ08} was given in \cite{GKV09}.

In this appendix we discuss the form and the most important analyticity properties of the solution 
of the asymptotic T-system for states when there are $N$ fundamental magnons with rapidities $u_j$ are present
in the system. These solutions correspond to the eigenvalues of the fusion hierarchy of the transfer matrices 
built from the S-matrices of the centrally extended  $SU(2|2)$ algebra such that the magnon rapidities
$u_j$ play the role of the inhomogeneities of the $SU(2|2)$ vertex model.

We introduce the following functions:
\begin{equation}
R_m(u)=\prod_{j=1}^{N} \, \frac{x(u)-x_j^+}{({x_j^+})^{\frac12}}, \qquad B_m(u)=\prod_{j=1}^{N} \, 
\frac{\frac{1}{x(u)}-x_j^+}{({x_j^+})^{\frac12}},    \label{RB_m}
\end{equation}
\begin{equation}
R_p(u)=\prod_{j=1}^{N} \, \frac{x(u)-x_j^-}{({x_j^-})^{\frac12}}, \qquad B_p(u)=\prod_{j=1}^{N} \, 
\frac{\frac{1}{x(u)}-x_j^-}{({x_j^-})^{\frac12}},
\end{equation}
where $x_j^{\pm}=x_s(u_j\pm \frac{i}{g})$. These functions satisfy the relation
\begin{equation}
R_m^+(u) \, B_m^+(u)=R_p^-(u) \, B_p^-(u)=(-1)^N \, Q(u),
\end{equation} 
with $Q(u)=\prod_{j=1}^{N} (u-u_j)$.

In case one is interested in states outside of the ${\alg{sl}(2)}$ sector then the auxiliary
Bethe roots appear in the formulae. To take into account their contribution as well, we
need to introduce the following functions:
\begin{equation}
R_l(u)=\prod_{j=1}^{K_l} \, \frac{x(u)-y_{l,j}}{(y_{l,j})^{\frac12}}, \qquad B_l(u)=\prod_{j=1}^{K_l} \, 
\frac{\frac{1}{x(u)}-y_{l,j}}{(y_{l,j})^{\frac12}}, \quad Q_l(u)=\prod_{j=1}^{K_l} (u-u_{l,j}), \quad l=1,2,3,
\end{equation}
where $y_{l,j}=x(u_{l,j})$ and they satisfy the relation
\begin{equation}
R_l(u) \, B_l(u)=(-1)^{K_l} \, Q_l(u), \qquad l=1,2,3.  \label{RBQl}
\end{equation}
The 3 family of Bethe roots $\{u_{l,j}\}_{l=1,2,3}$ correspond to the 3 levels of the $SU(2|2)$ nested Bethe
Ansatz.

Using the definitions above the asymptotic solution of the T-system is given by the formulae as follows.
\begin{equation}
T^{(0)}_{0,s}(u)=1, \qquad T^{(0)}_{a,0}(u)=1,    \label{T0sT0a0}
\end{equation} 
\begin{eqnarray}
T^{(0)}_{a,1}&=&(-1)^{a} \, \frac{Q_3^{[-a]} \, Q_1^{[a]}}{Q^{[a+1]}} \, \frac{B_p^{[a]}}{B_m^{[a]}} \,
\left \{  \frac{Q^{[1+a]}}{Q_1^{[a]} \, Q_3^{[a]}} \, \frac{B_m^{[a]}}{B_p^{[a]}}+ 
\frac{Q^{[1-a]}}{Q_3^{[-a]} \, Q_1^{[-a]}} \, \frac{B_m^{[-a]}}{B_p^{[-a]}}
\right. \nonumber \\
&+& \Theta(a-2) \, \sum_{n=0}^{a-2} \, \frac{Q^{[a-1-2n]}}{Q_3^{[a-2-2n]} \, Q_1^{[a-2-2n]}} \, 
\left( \frac{B_m^{[a-2-2n]}}{B_p^{[a-2-2n]}}+\frac{R_m^{[a-2-2n]}}{R_p^{[a-2-2n]}} \right) \label{Ta10} \\
&-& \Theta(a-1) \, \sum_{n=0}^{a-1}  
\left. \frac{Q^{[a-1-2n]}}{Q_3^{[a-2-2n]} \, Q_1^{[a-2n]} } \, \left(  
\frac{Q_1^{[a-2n]} \, Q_2^{[a-3-2n]}}{ Q_1^{[a-2-2n]} \, Q_2^{[a-1-2n]}}+
\frac{ Q_3^{[a-2-2n]} \, Q_2^{[a+1-2n]}}{ Q_3^{[a-2n]} \, Q_2^{[a-1-2n]}}  \right)\right\}, \nonumber
\end{eqnarray}
where $\Theta(x)$ is the unitstep function such that $\Theta(0)=1$. $T^{(0)}_{a,1}$ admit the eigenvalues of 
the transfer matrices corresponding to the anti-symmetric irreducible
representations of $SU(2|2)$ in the auxiliary space. The eigenvalues belonging to the symmetric
representations are given by:

\begin{eqnarray}
T_{1,s}^{(0)}&=&\frac{1}{Q_1^{[-s]} \, Q_3^{[s]}} \, \prod_{j=1}^{s-1} \frac{R_m^{[2j-s]}}{R_p^{[2j-s]}} \,
\left \{ Q_2^{[-s-1]} \, Q_2^{[s+1]} \, \frac{R_m^{[s]}}{R_p^{[s]}} \, \sum_{k=0}^{s} \, F_{s,k}
\right. \nonumber \\
&-& 
\Theta(s-1) \, \left( Q_2^{[s-1]} \, Q_2^{[-s-1]} \, \sum_{k=0}^{s-1} \, F_{s,k} 
-Q_2^{[1-s]} \, Q_2^{[s+1]} \, \frac{B_m^{[-s]}}{B_p^{[-s]}} \, \frac{R_m^{[s]}}{R_p^{[s]}} \,
\sum_{k=1}^{s} F_{s,k} \right) \nonumber \\
&+& \left. \Theta(s-2) \, Q_2^{[1-s]} \, Q_2^{[s-1]} \, \frac{B_m^{[-s]}}{B_p^{[-s]}} \, \sum_{k=1}^{s-1} \, %%@
F_{s,k}
\right \},    \label{T1s0}
\end{eqnarray}
where 
\begin{equation}
F_{s,k}=\frac{Q_1^{[2k-s]} \, Q_3^{[2k-s]}}{Q_2^{[2k-1-s]} \, Q_2^{[2k+1-s]} }. \label{Fsk}
\end{equation}
Finally T-functions on the interior boundaries of the fat-hook are given by:
\begin{equation}
T^{(0)}_{a,2}=\left(  {\cal{F}}^{(0)} \, \frac{R_m^-}{R_p^-} \, \frac{1}{Q^{[-2]}} \, \frac{Q_1^-}{Q_3^-} 
\right)^{[a]} 
\, \left( {\cal{G}}^{(0)} \, \frac{R_m^+}{R_p^+} \, Q^{[2]} \, \frac{Q_3^+}{Q_1^+} \right)^{[-a]}, \qquad a 
\geq 2 
\label{Ta20}
\end{equation}
\begin{equation}
T^{(0)}_{2,s}=\left(  {\cal{F}}^{(0)} \, \frac{R_p^-}{R_m^-} \, \frac{Q_1^-}{Q_3^-} \right)^{[s]} 
\, \left( {\cal{G}}^{(0)} \, \frac{R_m^+}{R_p^+} \, \frac{Q_3^+}{Q_1^+} \right)^{[-s]}  \,
\left( \prod_{k=1}^{s-1} \frac{R_m^{[2k+1-s]}}{R_p^{[2k+1-s]}} \right)^2, \qquad s \geq 2, \label{T2s0}
\end{equation}
where ${\cal{F}}^{(0) +}$ and ${\cal{G}}^{(0) -}$ are the analytical continuations of $T_{1,1}^{(0)}$ through 
the
branch cut at $\frac{i}{g}$ and $-\frac{i}{g}$ respectively.
\begin{equation}
{\cal{F}}^{(0)}=(T_{1,1}^{(0) +})_*^- ,\qquad {\cal{G}}^{(0)}=(T_{1,1}^{(0) -})_*^+.    \label{F0G0T11}
\end{equation}
They are given explicitely by: 
\begin{equation}
{\cal{F}}^{(0)}=-\frac{Q_3^{-}}{Q_3^{+}}+\frac{R_m^+}{R_p^+} \, 
\left( \frac{Q_2^{++} \, Q_3^-}{Q_2 \, Q_3^+} + \frac{Q_2^{--} \, Q_1^+}{Q_2 \, Q_1^-} \right)-
\frac{R_m^- \, R_m^+}{R_p^- \, R_p^+} \, \frac{Q_1^+}{Q_1^-}, \label{F0}
\end{equation}
\begin{equation}
{\cal{G}}^{(0)}=-\frac{Q_3^{-}}{Q_3^{+}}+\frac{B_m^+}{B_p^-} \, 
\left( \frac{Q_2^{++} \, Q_3^-}{Q_2 \, Q_3^+} + \frac{Q_2^{--} \, Q_1^+}{Q_2 \, Q_1^-} \right)-
\frac{B_m^- \, B_m^+}{B_p^- \, B_p^+} \, \frac{Q_1^+}{Q_1^-}.     \label{G0}
\end{equation}
The Bethe Ansatz equations follow from the fact that the residues of the poles of the 
transfer matrices coming from the functions $Q_l, \quad l=1,2,3$ are equal to zero:
\begin{equation}
\frac{Q_2^-(u_{1,j})}{Q_2^+(u_{1,j})} \frac{B_p (u_{1,j})}{B_m (u_{1,j})}=1, \qquad j=1,.., K_1
\label{BA1}
\end{equation}
\begin{equation}
\frac{Q_2^{++}(u_{2,j})}{Q_2^{--}(u_{2,j})}  \frac{Q_1^-(u_{2,j})}{Q_1^+(u_{2,j})}
\frac{Q_3^-(u_{2,j})}{Q_3^+(u_{2,j})}=-1, \qquad j=1,.., K_2
\label{BA2}
\end{equation}
\begin{equation}
\frac{Q_2^-(u_{3,j})}{Q_2^+(u_{3,j})} \frac{R_p(u_{3,j})}{R_m(u_{3,j})}=1, \qquad j=1,.., K_3.
\label{BA3}
\end{equation}

The analyticity properties of the asymptotic T-functions can be easily read off from the formulae
above. Now, we summarize their most important properties. $T^{(0)}_{a,1}$ has square root branch cuts
along the lines $\mbox{Im} u= \pm \frac{a}{g}$. ${\cal{F}}^{(0)}$ and ${\cal{G}}^{(0)}$ have square root branch 
cuts
along the lines $\mbox{Im} u= \pm \frac{1}{g}$.
From (\ref{T1s0}) it can be seen that $T_{1,s}^{(0)}$ has square root branch cuts between the lines
$\mbox{Im} u= \pm \frac{s}{g}$, but all these cuts are generated by a gauge transformation which cancels
from the Y-functions. Separating the gauge factor:
\begin{equation}
\tilde{T}^{(0)}_{1,s}=T^{(0)}_{1,s} \, \prod_{j=1}^{s-1} \frac{R_p^{[2j-s]}}{R_m^{[2j-s]}}, \label{T1s0tilde} 
\end{equation}
it can be seen that $\tilde{T}^{(0)}_{1,s}$ has discontinuities only along the lines $\mbox{Im} u= \pm \frac{s}{g}$. 

For our considerations another important analyticity information is the large $u$ behavior of the T-functions. 
Analysing the formulae above it turns out that imposing the level matching condition
 (i.e. $\sum_{j=1}^N \, u_j=0$):
\begin{equation}
T^{(0)}_{a,1}(u) \sim A^{(0)} \, \frac{a}{u^2} \qquad \quad \mbox{for} \quad |u| \rightarrow \infty \qquad %%@
a=1,2,...,
\end{equation} 
when $|\mbox{Im} u| < \frac{a}{g}$.  The coefficient $A^{(0)}=-\frac{\mu \, (\mu+2)}{g^2},$
where $\mu= i \, g\, \sum\limits_{j=1}^{N} \left( \frac{1}{x_j^+}-\frac{1}{x_j^-}  \right)$ is a real
and positive number.
 In the region $|\mbox{Im} u| > \frac{a}{g}$ there is a change in the large 
$u$ behavior of $T^{(0)}_{a,1}(u)$. There they decay only as $\frac{1}{u}$.

In the mirror TBA equations only the zeroes and poles of $T_{a,1}(u)$ and $T_{1,s}(u)$
located in the physical strip  (i.e the strip $\mbox{Im}u \leq \frac{1}{g}$)
furthermore the zeroes and poles of ${\cal{F}}^{+}$ and ${\cal{G}}^{-}$ on the upper and lower half
planes respectively are relevant. Though the asymptotic formulae presented above valid for a 
general state in this paper we considered states where $T_{1,1}$, ${\cal{F}}^+$ and ${\cal{G}}^-$
have no zeros and poles in the regions $|\mbox{Im} \, u|\leq 1/g$, $\mbox{Im} \, u \geq 0$ and $\mbox{Im} \, u 
< 0$ respectively. We believe (though not sure) that this condition is satisfied within
 the ${\alg{sl}(2)}$ sector of the theory. 

More presisely we derived the TBA equations to a subset of the ${\alg{sl}(2)}$ sector that we
called the ${\alg{sl}(2)}$ (sub-)sector. In this subsector there is a symmetry
between the left and right wing variables so we do not hang wing index to the variables. 
In the asymptotic limit the ${\alg{sl}(2)}$ (sub-)sector is characteried by the properties:
\begin{itemize}

\item $T^{(0)}_{1,1}$ has neither zeros nor poles in the physical strip.

%\item $T^{(0)}_{2,1}$ has  poles at positions $u_j-\frac{i}{g}$.

\item $T^{(0)}_{a,s}$ have no poles in the physical strip except $T^{(0)}_{2,1}$ which 
has  poles at positions $u_j-\frac{i}{g}  \qquad j=1,..,N$.

\item $T^{(0)}_{a,1}$ has only zeroes in the physical strip at positions $\xi_{a,j}^{(0)}$ 
for $a \geq 2$, and their contributions are taken into account by the factor
$\tau_{a}(u)=\prod\limits_{j=1}^{{\cal N}_{a}} t(u-\xi_{a,j}^{(0)})$.
 
\item $\tilde{T}^{(0)}_{1,s}$ has only zeroes in the physical strip at positions $\tilde{\xi}_{s,j}^{(0)}$ 
for $s \geq 2$, and their contributions are taken into account by the factor
$\tilde{\tau}_{s}(u)=\prod\limits_{j=1}^{\tilde{\cal N}_{s}} t(u-\xi_{s,j}^{(0)})$.

\item There are no zeroes located at the boundaries of the physical srtip, namely with imaginary part
$\pm 1/g$.

\item ${\cal{F}}^{(0) +}$ has neither zeros nor poles it the region $\mbox{Im} u \geq 0$.

\item ${\cal{G}}^{(0) -}$ has neither zeros nor poles it the region $\mbox{Im} u<0$.

\end{itemize}
We just recall that $\tau_1(u)=\prod\limits_{j=1}^{{ N}} t(u-u_j)$ .%and mention that all the poles located 
%in the physical strip are given by the 2nd property since there are no poles
%the existence of other poles 
% is excluded by the Bethe equations (\ref{BA1}-\ref{BA3}).
In the ${\alg{sl}(2)}$ (sub-)sector the source terms appearing in the TBA equations (\ref{TBAmvw}-\ref{TBA-}) 
can be expressed in terms of the $\tau_m$ and $\tilde{\tau}_{m}$ functions as follows:
\begin{eqnarray}
t_{m \vert vw}&=&\tau_m \tau_{m+2}, \qquad m=1,2,... \label{tmvw}\\
t_{m \vert w}&=&\tilde{\tau}_m \tilde{\tau}_{m+2}, \qquad m=1,2,... \label{tmw}\\
t_Q&=& \tau_Q^2, \qquad Q=2,3,... \label{tQ}\\
t_1&=&1 \label{t1}\\
t_{-}&=&\tau_2 /\tilde{\tau}_2, \label{t-}
\end{eqnarray}
where because of the left right symmetry we have omitted the upper case $(\alpha)$ index.

The class of minimal energy twist-two states forms an important subset within the ${\alg{sl}(2)}$ (sub-)sector. 
Because of the importance of these states we studied numerically the qualitaive analyticity properties of the
$T$-functions of this class. These can be summarized as follows:
\begin{itemize}

\item $T^{(0)}_{1,1}$ has neither zeros nor poles in the physical strip,

\item $T^{(0)}_{2,1}$ has $2(N-2)$ zeros on the real axis and poles at positions $u_j-\frac{i}{g}$,

\item $T^{(0)}_{a,1}$ has $2(N-2)$ zeros on the real axis for $a \geq 3$,
 
\item $\tilde{T}^{(0)}_{1,s}$ has neither zeros nor poles in the physical strip,

\item ${\cal{F}}^{(0) +}$ has neither zeros nor poles it the region $\mbox{Im} u \geq 0$,

\item ${\cal{G}}^{(0) -}$ has neither zeros nor poles it the region $\mbox{Im} u<0$.

\end{itemize}
Near the small coupling limit all the magnon rapidities and the real zeroes of $T_{a,1}$ are larger than 2, 
because they are of order $\frac{1}{g}$.

 The previously summarized analyticity properties of the asymptotic T-functions determine the
 analyticity properties for the asymptotic Y-functions through the formula (\ref{YT}). 
Their state independent anayticity properties can be summarized as follows.
 $Y_{a,1}^{(0)}$ and $Y_{1,s}^{(0)}$ tends to a constant at infinity and they have square root branch cuts
 along the lines $\mbox{Im} u =  \pm (a \pm 1)$ and $\mbox{Im} u =  \pm (s \pm 1)$ respectively.
 $Y_{11}^{(0)}$ and $Y_{22}^{(0)}$ tend to $-1$ at infinity and have square root branch cuts along the lines
 $\mbox{Im} u=0,\pm 2$, such that $1+Y_{11}^{(0)} \sim 1/u$ and $1+\frac{1}{Y_{22}^{(0)}} \sim 1/u$
at the infinity. 
 
The state dependent analyticity properties such as the distribution of zeroes and poles can be read off
from the local singularity structure of the corresponding T-functions studied above. 
 

\subsection{Asymptotic solution for the momentum carrying nodes}

In the asymptotic limit the Y-system decouples to two $SU(2|2)$ T-systems. Correspondingly
we will hang an L (left) and an R (right) indexes to the asymptotic transfer matrices. 
Then the asymptotic solution for the momentum carrying nodes takes the form \cite{GKV09}:
\begin{equation} \label{Ya00}
Y_{a,0}^{(0)}=\left( \frac{x^{[a]}}{x^{[-a]}} \right)^{J_{eff}} \, {\cal{D}}_a 
\,\frac{B_{1,L}^{[-a]}}{B_{1,L}^{[a]}} \, \frac{B_{3,L}^{[a]}}{B_{3,L}^{[-a]}}
\,\frac{B_{1,R}^{[-a]}}{B_{1,R}^{[a]}} \, \frac{B_{3,R}^{[a]}}{B_{3,R}^{[-a]}} \,
T^{(0) L}_{a,-1} \,T^{(0) R}_{a,1} \qquad a=1,2,...,  
\end{equation}
where $J_{eff}=J+\frac{K_{3,L}-K_{1,L}+K_{3,R}-K_{1,R}}{2}$ and the factor ${\cal{D}}_a $
contains the dressing phase of fundamental magnons as follows.
%(Ez mar a dressing phase vagasait megado appendix utan kell)
Let: 
\begin{equation}
{\cal{D}}_1(u)=\frac{B_m^-(u) \, R_p^+(u)}{B_p^+ (u)\, R_m^-(u)} \, 
\prod\limits_{j=1}^N e^{-2 \, i\, \theta(u,u_j)} \equiv \prod\limits_{j=1}^N S_{\alg{sl}(2)}^{1 1_*}(u,u_j),
\end{equation}
with $\theta(u,u_j)$ given by (\ref{theta}). 
%(dressing vagasait megado fejezebeli keplet, lenyeg mirror-fizikai thetak produktuma)
Then
\begin{equation}
{\cal{D}}_a(u)=\prod_{k=0}^{a-1} \, {\cal{D}}_1^{[a-1-2k]}(u) \equiv 
\prod\limits_{j=1}^N S_{\alg{sl}(2)}^{a 1_*}(u,u_j).
\end{equation}
In the ${\alg sl}(2)$ sector the following representation for $Y_{1,0}^{(0)}$ proved to be useful:
\begin{eqnarray}
Y_{1,0}^{(0)}=Y_{d}^{(0)} \, T_{1,1}^{L} \, T_{1,1}^{R}, \qquad Y_{d}^{(0)}=y_d,
\end{eqnarray} 
where $y_d$ contains the dressing part of $Y_{1,0}^{(0)}$:
\begin{equation}
y_d=\left(\frac{x^+}{x^-}\right)^J \, {\cal D}_1.
\label{yd}
\end{equation}
The Beisert-Staudacher equations follow from the requirement that $Y^{(0)}_{1,0 (*)}(u_k)=-1$, where
$Y^{(0)}_{1,0 (*)}=\left((Y^{(0) -}_{1,0})_*\right)^+$.
In words $Y^{(0)}_{1,0}(u)$ analytically continued through the branch cut at $-\frac{i}{g}$
to the physical sheet and taken at the positions of the physical rapidities is equal to $-1$.
Starting from (\ref{Ya00}) this analytical continuation can be implemented simply by using (\ref{F0G0T11}) and 
(\ref{G0}). The equations take the form:
\begin{equation}
\left( \frac{x_s^{+}}{x_s^{-}} \right)^{J_{eff}}  S_{\alg{sl}(2)} \,
\,\frac{B_{1,L}^{-}}{R_{1,L}^{+}} \, \frac{R_{3,L}^{-}}{B_{3,L}^{+}}
\,\frac{B_{1,R}^{-}}{R_{1,R}^{+}} \, \frac{R_{3,R}^{-}}{B_{3,R}^{+}}
\bigg|_{u_k} =-1, \qquad j=1,..,N,
\end{equation}
where we introduced the notation $S_{\alg{sl}(2)}(u)=\prod\limits_{j=1}^N S_{\alg{sl}(2)}^{1_* 1_*}(u,u_j)$ for %%@
short.
For states outside of the ${\alg{sl}(2)}$ sector there are 6 other bethe equations that can be obtained by
hanging $L$ and $R$ indices to the 3 auxiliary Bethe equations (\ref{BA1})-(\ref{BA3}).

We close the appendix by the discussion of the analyticity properties of $Y_{a,0}^{(0)}$.
 They have square root branch cuts along the lines $\mbox{Im} u =\pm \frac{a}{g}$. 
They do not have zeros on the complex plane and the distribution of poles is as follows.
\begin{itemize}
\item $Y_{1,0}^{(0)}$ has poles at positions $u_j^{[\pm 2]}$,
\item $Y_{a,0}^{(0)}$ has poles at positions $u_j^{[\pm(a-1)]}$ and $u_j^{[\pm(a+1)]} \qquad a=2,3...$.
\end{itemize}

For large $u$ the $Y_{a,0}^{(0)}$ behaves like:
\begin{eqnarray}
Y_{a,0}^{(0)}(u) \sim  
{1 \over u^{2(J+2+N+\mu)}}, \qquad \mbox{for} \qquad \mbox{Im} u \leq \frac{a}{g}, 
\nonumber
\end{eqnarray}
and tends to a constant when $\mbox{Im} u > \frac{a}{g}$. 

%For large $u$ the $Y_{a,0}^{(0)}$ behaves like:
%\begin{eqnarray}
%Y_{a,0}^{(0)}(u) \sim \frac{1}{u^{2(J+2+N+\mu)}}, \qquad \mbox{for} \qquad \mbox{Im u} \leq \frac{a}{g}, 
%\nonumber \\
%Y_{a,0}^{(0)}(u) \sim \mbox{constant}, \qquad \mbox{for} \qquad \mbox{Im u} > \frac{a}{g}.
%\end{eqnarray}


The formulae and properties of the asymptotic solution summarized in this appendix provided
with the qualitative analticity information which made possible the derivation of the TBA equations
for the exact energies. 



==> nzbib <==

\begin{thebibliography}{999}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%1
\bibitem{adscft} J.~M.~Maldacena,
``The large N limit of superconformal field theories and supergravity,''
Adv.\ Theor.\ Math.\ Phys.\  {\bf 2} (1998) 231
[Int.\ J.\ Theor.\ Phys.\  {\bf 38} (1999) 1113], [hep-th/9711200];\\
S.~S.~Gubser, I.~R.~Klebanov and A.~M.~Polyakov,
``Gauge theory correlators from non-critical string theory,''
Phys.\ Lett.\ B {\bf 428} (1998) 105, [hep-th/9802109];\\
E.~Witten,
``Anti-de Sitter space and holography,''
Adv.\ Theor.\ Math.\ Phys.\  {\bf 2} (1998) 253, [hep-th/9802150].
%3
\bibitem{S}
M.~Staudacher, ``The factorized S-matrix of CFT/AdS",
JHEP{\bf 05} (2005) 054  [arXiv:hep-th/0412188];
\\
R.~Janik, ``The $\text{AdS}_5\times\text{S}^5$ superstring
worldsheet S-matrix and crossing symmetry", Phys. Rev. {\bf D73}
(2006) 086006 [arXiv:hep-th/0603038];
\\
N.~Beisert, R.~Hernandez and  E.~Lopez, ``A crossing symmetric phase
for $\text{AdS}_5\times\text{S}^5$ strings", JHEP{\bf 11} (2006) 070
[arXiv:hep-th/0609044]; 
\\
N.~Beisert, B.~Eden and  M.~Staudacher,
``Transcendentality and crossing",
J.\ Stat.\ Mech.\  {\bf 0701} (2007) P021
[arXiv:hep-th/0610251];
\\
N.~Beisert,
``The su(2|2) dynamic S-matrix",
Adv.\ Theor.\ Math.\ Phys.\  {\bf 12} (2008) 945
[arXiv:hep-th/0511082];
%4
\bibitem{dressing}
N.~Dorey, D.M.~Hofman and J.M.~Maldacena,
``On the singularities of the magnon S-matrix'',
Phys.\ Rev.\  D {\bf 76}, 025011 (2007)
[arXiv:hep-th/0703104].  \\
D.~Volin,
``Minimal solution of the AdS/CFT crossing equation,''
J.\ Phys.\ A  {\bf 42}, 372001 (2009)
[arXiv:0904.4929 [hep-th]].
%5
\bibitem{dresscross}
G. Arutyunov, S. Frolov,
``The dressing factor and crossing equations'',
J.\ Phys.\ A  {\bf 42}, 425401 (2009)
[arXiv:0904.4575 [hep-th]].
%2
\bibitem{BS}
  N.~Beisert and M.~Staudacher,
  ``Long-range PSU(2,2$|$4) Bethe ansaetze for gauge theory and strings,''
  Nucl.\ Phys.\ B {\bf 727}, 1 (2005)
  [hep-th/0504190].
%55
\bibitem{S1}
 C. Ahn and R. I. Nepomechie, "Exact world-sheet S-matrix", [arxiv:1012.3991 [hep-th]].
 %56 
\bibitem{S2}
 P. Vieira and D. Volin, "The dressing factor", [arxiv:1012.3992 [hep-th]].
 %9
\bibitem{Luscher85}
  M.~Luscher,
  ``Volume Dependence of the Energy Spectrum in Massive Quantum Field Theories. 1. Stable Particle States,''
 {\slshape   Commun.\ Math.\ Phys.\  }{\bf 104} (1986) 177.
%8
\bibitem{JL07}
  R.~A.~Janik and T.~Lukowski,
  ``Wrapping interactions at strong coupling -- the giant magnon,''
 {\slshape   Phys.\ Rev.\  D }{\bf 76} (2007) 126008
  [arXiv:0708.2208 [hep-th]].
%7
\bibitem{BJ08}
  Z.~Bajnok and R.~A.~Janik,
  ``Four-loop perturbative Konishi from strings and finite size effects for multiparticle states,''
 {\slshape   Nucl.\ Phys.\  B }{\bf 807} (2009) 625
  [arXiv:0807.0399 [hep-th]].
%10
\bibitem{Sieg}
  F.~Fiamberti, A.~Santambrogio, C.~Sieg and D.~Zanon,
  ``Wrapping at four loops in N=4 SYM,''
  Phys.\ Lett.\  B {\bf 666} (2008) 100
  [arXiv:0712.3522 [hep-th]].
%11  
\bibitem{Vel}
  V.~N.~Velizhanin,
  ``The Four-Loop Konishi in N=4 SYM,''
  arXiv:0808.3832 [hep-th].
%12
\bibitem{Bajnok:2008qj}
  Z.~Bajnok, R.~A.~Janik and T.~Lukowski,
  ``Four loop twist two, BFKL, wrapping and strings,''
  Nucl.\ Phys.\  B {\bf 816} (2009) 376
  [arXiv:0811.4448 [hep-th]].
%15
\bibitem{BJ09}
  Z.~Bajnok, A.~Hegedus, R.~A.~Janik and T.~Lukowski,
  ``Five loop Konishi from AdS/CFT,''
  Nucl. Phys. B {\bf 827} (2010), 426-456,
  arXiv:0906.4062 [hep-th].
%16
\bibitem{Lukowski:2009ce}
  T.~Lukowski, A.~Rej and V.~N.~Velizhanin,
  ``Five-Loop Anomalous Dimension of Twist-Two Operators,''
  Nucl.Phys.B {\bf 831}   (2010), 105-132,
  arXiv:0912.1624 [hep-th].
%13
\bibitem{KL02}
A.~V.~Kotikov and L.~N.~Lipatov,
``DGLAP and BFKL Evolution Equations in the ${\mathcal{N}}\!=4$ Supersymmetric Gauge   Theory,''
Nucl.\ Phys.\  B {\bf 661} (2003) 19
[Erratum-ibid.\  B {\bf 685} (2004) 405]
[arXiv:hep-ph/0208220].
%14
\bibitem{40_5}
  A.~V.~Kotikov, L.~N.~Lipatov, A.~Rej, M.~Staudacher and V.~N.~Velizhanin,
  ``Dressing and Wrapping,''
  J.\ Stat.\ Mech.\  {\bf 0710} (2007) P10003
  [arXiv:0704.3586 [hep-th]].
%61
\bibitem{Zami}
Al.B. Zamolodchikov, "Thermodynamic Bethe ansatz in relativistic models. Scaling three
state Potts and Lee-Yang models", Nucl. Phys. B 342, 695 (1990).
%6
\bibitem{AJK}
  J.~Ambjorn, R.~A.~Janik and C.~Kristjansen,
  ``Wrapping interactions and a new source of corrections to the spin-chain / string duality,''
 {\slshape   Nucl.\ Phys.\  B }{\bf 736} (2006) 288
  [arXiv:hep-th/0510171].
%17  
\bibitem{AF07}
  G.~Arutyunov and S.~Frolov,
  ``On String S-matrix, Bound States and TBA,''
  JHEP {\bf 0712} (2007) 024, hep-th/0710.1568.
%18
\bibitem{AF09a}
  G.~Arutyunov and S.~Frolov,
  ``String hypothesis for the $AdS$ mirror,''
  JHEP {\bf 0903} (2009) 152
  [arXiv:0901.1417 [hep-th]].
%21
\bibitem{Bombardelli:2009ns}
  D.~Bombardelli, D.~Fioravanti and R.~Tateo,
  ``Thermodynamic Bethe Ansatz for planar AdS/CFT: a proposal,''
  J.\ Phys.\ A  {\bf 42} (2009) 375401
  [arXiv:0902.3930].
%19  
\bibitem{AF09b}
  G.~Arutyunov and S.~Frolov,
  ``Thermodynamic Bethe Ansatz for the $AdS$ Mirror Model,''
  JHEP {\bf 0905} (2009) 068
  [arXiv:0903.0141 [hep-th]].
%22
\bibitem{GKKV09}
  N.~Gromov, V.~Kazakov, A.~Kozak and P.~Vieira,
  ``Exact Spectrum of Anomalous Dimensions of Planar N = 4 Supersymmetric
   Yang-Mills Theory: TBA and excited states,''
  Lett.Math.Phys.91:265-287,2010, [arXiv:0902.4458v3 [hep-th]].
%20
\bibitem{AF09d}
  G.~Arutyunov and S.~Frolov,
  ``Simplified TBA equations of the $AdS_5 \times S^5$ mirror model,''
  JHEP 0911:019,2009, arXiv:0907.2647 [hep-th].
%30
\bibitem{GKV09}
  N.~Gromov, V.~Kazakov and P.~Vieira,
  ``Integrability for the Full Spectrum of Planar AdS/CFT,''
  Phys.Rev.Lett.103:131601,2009, arXiv:0901.3753 [hep-th].
%35
\bibitem{KPS}
A. Kl\"umper, P.A. Pearce, 
"Analytic calculation of scaling dimensions: Tricritical hard squares and critical hard hexagons",
J. Stat. Phys 64 (1991) 13-76; 
"Conformal weights of RSOS lattice models and their fusion hierarchies", 
Physica A183 (1992) 304-350. 
%36
\bibitem{33B}
A. Kuniba, K. Sakai and J. Suzuki, 
"Continued fraction TBA and functional relations in XXZ model at root of unity",
Nucl. Phys. B525 [FS] (1998) 597, [arXiv:math/9803056].
%23
\bibitem{DT}
P. Dorey, R. Tateo, "Excited states by analytic continuation of TBA equations," Nucl.
Phys. B 482, 639 (1996) [arXiv:hep-th/9607167]. 
%42
\bibitem{BLZ}
V.V. Bazhanov, S. Lukyanov, A.B. Zamolodchikov, 
"Integrable Structure of Conformal Field Theory II. Q-operator and DDV equation",
Comm. Math. Phys. 190 (1997) 247, [arXiv:hep-th/9604044];
"Integrable Quantum Field Theories in Finite Volume: Excited State Energies",
Nucl. Phys. B489 (1997) 487, [arXiv:hep-th/9607099].
%38
\bibitem{BH-SG}
J. Balog, \'A. Heged\H{u}s, 
"TBA equations for excited states in the Sine-Gordon model",
 J. Phys. A37 (2004) 1903, [arXiv:hep-th/0304260]
%39
\bibitem{BH34}
J. Balog, \'A. Heged\H{u}s, 
"TBA equations for excited states in the O(3) and O(4) nonlinear $\sigma$-model", 
 J. Phys. A37 (2004) 1881, [arXiv:hep-th/0309009]
%24
\bibitem{GKV09b}
  N.~Gromov, V.~Kazakov and P.~Vieira,
  ``Exact AdS/CFT spectrum: Konishi dimension at any coupling,''
  Phys.Rev.Lett.104:211601,2010, [arXiv:0906.4240 [hep-th]].
%25
\bibitem{Arutyunov:2009ax}
  G.~Arutyunov, S.~Frolov and R.~Suzuki,
  ``Exploring the mirror TBA,''
  JHEP 1005:031,2010, [arXiv:0911.2224 [hep-th]].
%26
\bibitem{Gromov}
  N.~Gromov,
  ``Y-system and Quasi-Classical Strings,''
  JHEP 1001:112,2010, [arXiv:0910.3608 [hep-th]].
%27
\bibitem{ujKazi}
N. Gromov, V. Kazakov, Z. Tsuboi,
"$PSU(2,2|4)$ character of quasiclasical AdS/CFT"
JHEP 1007:097,2010, [arXiv:1002.3981 [hep-th]].
%57
\bibitem{Frolnum}
S. Frolov,
"Konishi operator at intermediate coupling",
 J.Phys.A{\bf 44}:065401,2011, [arXiv:1006.5032 [hep-th]]. 
%62
\bibitem{StrongKonishi}
N. Gromov, D. Serban, I. Shenderovich and D. Volin, "Quantum folded string and integrability:
 from finite size effects to Konishi dimension", [arXiv:1102.1040[hep-th]], \\
R. Roiban and A. A. Tseytlin, "Semiclassical string computation of strong-coupling
corrections to dimensions of operators in Konishi multiplet", 
[arXiv:1102.1209 [hep-th]]  \\
B. C. Vallilo and L. Mazzucato, "The Konishi multiplet at strong coupling", 
 [arXiv:1102.1219 [hep-th]].
%28
\bibitem{AFS}
G.~Arutyunov, S.~Frolov and R.~Suzuki,
``Five-loop Konishi from the Mirror TBA'',
JHEP 1004:069,2010,  [arXiv:1002.1711 [hep-th]].
%50
\bibitem{BH-BJ}
J. Balog, \'A. Heged\H{u}s, "The Bajnok-Janik formula and wrapping corrections",
JHEP 1009:107,2010,  [arXiv:1003.4303 [hep-th]]. 
%51
\bibitem{BHxxx}
J. Balog, \'A. Heged\H{u}s, "5-loop Konishi from linearized TBA and the XXX magnet",
JHEP 1006:080,2010, [arXiv:1002.4142 [hep-th]].
%52
\bibitem{Tateo1}
A. Cavaglia, D. Fioravanti, R. Tateo,  "Extended Y-system for the $AdS_5/CFT_4$ correspondence", 
 Nucl.Phys. B {\bf 843}, (2011) 302-343, [arXiv:1005.3016 [hep-th]].
%53
\bibitem{Tateo2}
A. Cavaglia, D. Fioravanti, M. Mattelliano, R. Tateo, "On the $AdS_5/CFT_4$ TBA and its analytic properties",
[arXiv:1103.0499 [hep-th]]. 
%54
\bibitem{Tateo3}
A. Cavaglia, D. Fioravanti, M. Mattelliano, R. Tateo, in preparation.
%60
\bibitem{devegasum}
H.J. De Vega, "Yang-Baxter Algebras, Integrable Theories and Quantum Groups", 
  Int.J.Mod.Phys.A4:2371-2463,1989. 
%58 
\bibitem{FR} 
 L. D. Faddeev, N. Yu. Reshetikhin, 
 "Integrability of the principal chiral field model in 1 + 1 dimension",
 Ann. Phys. 167 (1986) 227-256; \\
 A. M. Polyakov, P. B. Wiegmann, 
 "Theory of nonabelian goldstone bosons in two dimensions",
 Phys. Lett. B131, (1984)  121-126; \\
H. M. Babujian, A. M. Tsvelick, 
"Heisenberg magnet with an arbitrary spin and anisotropic chiral field ",
 Nucl. Phys. B265 [FS15] (1986) 24-44.
%59
\bibitem{LC}
 C. Destri, H.J. de Vega, 
"Light Cone Lattice Approach To Fermionic Theories In 2-D: The Massive Thirring Model",
Nucl.Phys.B{\bf 290}:363,1987. \\
C. Destri, H.J. de Vega, "Integrable Quantum Field Theories And Conformal Field Theories From Lattice Models In 
The Light Cone Approach", Phys.Lett.B201:261,1988,  \\
C. Destri, H.J. de Vega,
"Light Cone Lattices And The Exact Solution Of Chiral Fermion And Sigma Models",
J.Phys.A22:1329,1989. 
%63 
\bibitem{Tquant}
S. Frolov, R. Suzuki,
"Temperature quantization from the TBA equations".
 Phys.Lett.B{\bf 679}:60-64,2009, [arXiv:0906.0499 [hep-th]].
%64
\bibitem{AFrev}
  G.~Arutyunov and S.~Frolov,
  ``Foundations of the $AdS_5 \times S^5$ Superstring. Part I,''
  J.\ Phys.\ A  {\bf 42} (2009) 254003
  [arXiv:0901.4937 [hep-th]].
%65
\bibitem{KL10}
V. Kazakov, S. Leurent,
''Finite Size Spectrum of SU(N) Principal Chiral Field from Discrete Hirota Dynamics'',
[arXiv:1007.1770 [hep-th]] 
%66
\bibitem{GKLT}
N. Gromov, V. Kazakov, S. Leurent, Z. Tsuboi,
''Wronskian Solution for AdS/CFT Y-system'',
 JHEP 1101:155,2011,  [arXiv:1010.2720 [hep-th]].
%67
\bibitem{RyoHybrid}
R. Suzuki
''Hybrid NLIE for the Mirror $AdS_5 x S^5$'',
[arXiv:1101.5165 [hep-th]].    








\end{thebibliography}


















==> nzdelta <==
In this section we determine the $\Delta$ discontinuity using the
relations (\ref{Deltacut}) and the corresponding dispersion relation.
At the same time we complete the construction of the T-system elements
we started in section 4. Our aim is to construct T-system elements that
are smooth deformations (similarly to the Y-system elements) of the 
corresponding asymptotic variables. As we have seen in section 4, this is
possible only partially. If, for example, $T_{a,1}$ is close to the
corresponding asymptotic $T_{a,1}^{(0)}$ solution for the right hand side of 
the diagram, then, in general, even for the left-right symmetric 
${\alg{sl}(2)}$ cases, $T_{a,-1}$ can be very different from the corresponding
asymptotic T-system elements on the left hand side of the diagram. We will 
work in this gauge which we call the R-gauge and when we want to emphasize 
this asymmetry we also use the notation $T^R_{a,s}$ for $T_{a,s}$. Of course, 
there also exists an analogous L-gauge, with corresponding T-system elements 
$T^L_{a,s}$, which are close to the asymptotic solution on the left hand side.

We start the calculation by writing
\begin{equation}
Y_1=Y_{1,0}=\frac{T_{1,1}T_{1,-1}}{T_{2,0}}=
\frac{T^R_{1,1}\,T^R_{1,-1}}{T_{2,0}}=Y_d\,T^R_{1,1}\,T^L_{1,-1}.
\label{dRL}
\end{equation}
The new object here is
\begin{equation}
Y_d=\frac{1}{T_{2,0}}\,\frac{T^R_{1,-1}}{T^L_{1,-1}}=\frac{t_{1,-1}}
{T_{2,0}},
\end{equation}
where $t_{a,s}=\frac{T^R_{a,s}}{T^L_{a,s}}$ is the gauge transformation
connecting the two gauges defined above. Corresponding to the three factors
in the last expression in (\ref{dRL}) we write
\begin{equation}
\Delta=\ln\frac{Y_1^+}{(Y^+_1)_*}=\Delta_R+\Delta_L+\Delta_3,
\end{equation}
where
\begin{equation}
\Delta_R=\ln\frac{(T^R_{1,1})^+}{((T^R_{1,1})^+)_*},\qquad
\Delta_L=\ln\frac{(T^L_{1,-1})^+}{((T^L_{1,-1})^+)_*},\qquad
\Delta_3=\ln\frac{Y_d^+}{(Y_d^+)_*}=\ln\frac{t_{1,-1}^+}{(t^+_{1,-1})_*}.
\end{equation}
We now rewrite the relation (\ref{Deltacut}), using also the results
of the previous section in the form
\begin{equation}
[\Delta]_{\pm 2N}=D^{(\pm2N)}_{12R}+D^{(\pm2N)}_{12L}\pm 
2(j^{[\epsilon]}+j^{[\epsilon]}_{{\rm red}}),
\label{Deltacut12RL}
\end{equation}
where
\begin{equation}
D^{(\pm2N)}_{12R}=\pm\left[\Lambda^{(+)}_\mp\right]_{\pm2N}
\pm\sum_{m=1}^N\left[\Lambda^{(+)}_m\right]_{\pm(2N-m)},\quad
D^{(\pm2N)}_{12L}=\pm\left[\Lambda^{(-)}_\mp\right]_{\pm2N}
\pm\sum_{m=1}^N\left[\Lambda^{(-)}_m\right]_{\pm(2N-m)}
\label{D12RL}
\end{equation}
and
\begin{equation}
\Lambda_\pm^{(\alpha)}=\ln\left(1-\frac{1}{Y^{(\alpha)}_\pm}\right),\qquad
\Lambda_m^{(\alpha)}=\ln\left(1+\frac{1}{Y^{(\alpha)}_{m\vert vw}}\right).
\end{equation}

So far (except the construction of the T-system elements in 
section~4) our considerations are valid for any state of the model.
From now on, for simplicity, we restrict our attention to states in the 
${\alg{sl}(2)}$ (sub-)sector defined in appendix A. We think that our methods
can straightforwardly be generalized to generic states, but some of the
subsequent formulae are considerably more complicated in the general case. 
Since the two sides are identical  in this special case, in the rest of
the paper we can omit the upper index $^{(\alpha)}$ of the Y-functions
$Y_\pm^{(\alpha)}$, $Y_{m\vert vw}^{(\alpha)}$ or $Y_{m\vert w}^{(\alpha)}$.

In the ${\alg{sl}(2)}$ (sub-)sector in the asymptotic limit we have
\begin{equation}
Y_d^{(0)}=y_d\,\qquad \Delta_3^{(0)}=\frac{y_d^+}{(y_d^+)_*}=\Delta_d
\end{equation}
and
\begin{equation}
[\Delta_3^{(0)}]_{\pm2N}=[\Delta_d]_{\pm2N}=\pm2j^{[\epsilon]},
\end{equation}
as discussed in appendix B.

The main part of the calculation is to determine (omitting the upper 
index $R$ of the T-functions)
\begin{equation}
\Delta_R=\ln\frac{T^+_{1,1}}{{\cal F}^+}.
\end{equation}
Note that $\Delta_R(u)=p(u)$, the discontinuity which was left undetermined 
in section 4. 

Considerable simplification occurs if we express $D^{(\pm2N)}_{12R}$
in terms of the T-system elements. For the upper sign we find
\begin{equation}
D^{(2N)}_{12R}=[\ln T^+_{1,1}]_{2N}+[\ln T_{N+1,1}]_{N-1}
-[\ln T_{N+2,1}]_N.
\end{equation}
In the gauge we are using $T_{a,1}$ are meromorphic functions in the
strip $(-a,a)$, which means that this simplifies to
\begin{equation}
D^{(2N)}_{12R}=[\ln T^+_{1,1}]_{2N}.
\end{equation}
Next we further specify our gauge: we require that ${\cal F}^+$ has no
discontinuities in the upper half plane. This is satisfied by the
asymptotic function ${\cal F}^{(0)+}$. We then have
\begin{equation}
D^{(2N)}_{12R}=\left[\ln \frac{T^+_{1,1}}{{\cal F}^+}\right]_{2N}
=[\Delta_R]_{2N}.
\label{disc12R}
\end{equation}
This relation above is in the sense of a discontinuity relation. In this sense
one has for any function $f$ and $q$
\begin{equation}
\left[\ln\frac{f}{q}\right]_Z=[\ln f]_Z,
\end{equation}
provided $q$ is meromorphic around the cut $Z$. However, as explained in
section 2, in the sense of dispersion relation we have for example
\begin{equation}
\int_2^\infty{\rm d}v[\ln^\prime f]_Z(v)=
\int_2^\infty{\rm d}v[\ln^\prime f(v+\frac{iZ}{g}+i\epsilon)
-\ln^\prime f(v+\frac{iZ}{g}-i\epsilon)]
\end{equation}
and the result will be different if we use $f/q$ instead of $f$ when
the meromorphic function $q$ has zeroes/poles on the cut. The correct
interpretation of the original relation (\ref{Deltacut}) can be found
out from the asymptotic limit of the relation and we find that 
this subtlety is relevant for the $N=1$ case only and in that relation
we have to make the substitution $\Lambda_1\Rightarrow\frac{\Lambda_1}
{p_2^-}$, where $p_2$ is a polynomial whose roots are the real zeroes
of $T_{2,1}$. Actually, an equivalent (and simpler) way of taking into 
account this effect is to simply omit the contribution of these poles 
from the dispersion relation.

Repeating the same calculation for the lower sign we find
\begin{equation}
D^{(-2N)}_{12R}=-[\ln {\cal G}^-+\ln{\cal F}^+-\ln T^+_{1,1}]_{-2N}
-[\ln T_{N+1,1}]_{-(N-1)}
+[\ln T_{N+2,1}]_{-N}.
\end{equation}
Note that the first term is obtained from
\begin{equation}
1-\frac{1}{Y_+}=1-\frac{1}{(Y_-)_*}=
1+(Y_{1,1})_*=\frac{(T_{1,1}^+)_*\,(T^-_{1,1})_*}{(T_{2,1})_*}=
\frac{{\cal F}^+\,{\cal G}^-}{T_{2,1}}.
\end{equation}
Adding to the list of gauge fixing conditions the requirement that
${\cal G}^-$ has no discontinuities in the lower half plane (satisfied
by the asymptotic ${\cal G}^{(0)-}$) and using the properties of
the $T_{a,1}$ functions we have for both signs
\begin{equation}
D^{(\pm2N)}_{12R}=\left[\ln \frac{T^+_{1,1}}{{\cal F}^+}\right]_{\pm2N}
=[\Delta_R]_{\pm2N}.
\label{disc12Rpm}
\end{equation}
(With the understanding that the correct way of transforming the 
discontinuity relations into dispersion relations means that we have to 
omit the contributions of real zeroes in the $N=1$ case.)

Since in the ${\alg{sl}(2)}$ (sub-)sector the two sides of the problem are identical
(in the language of Y-functions) we have
\begin{equation}
[\Delta]_{\pm2N}=2D^{(\pm2N)}_{12R}\pm2(j^{[\epsilon]}
+j_{{\rm red}}^{[\epsilon]})
\end{equation}
and using (\ref{disc12Rpm}) this simplifies to
\begin{equation}
[\Delta_3]_{\pm2N}=\pm2(j^{[\epsilon]}+j_{{\rm red}}^{[\epsilon]}).
\end{equation}
We now define $Z_d$ and find the relations
\begin{equation}
Y_d=y_d\,Z_d,\qquad
\Delta_3=\Delta_d+\Delta_{{\rm red}},\qquad
\Delta_{{\rm red}}=\ln\frac{Z_d^+}{(Z_d^+)_*}.
\end{equation}

Since asymptotically $Z_d^{(0)}=1$, $\Delta_{{\rm red}}^{(0)}=0$ we conclude 
that in the exact solution ${\rm e}^{\Delta_{{\rm red}}}$ has no zeroes/poles
(and has constant asymptotics for large $\vert u\vert$). This means that if
we define (analogously to $\Gamma^{(\alpha)}(u)$ of section~5)
\begin{equation}
\Gamma_{{\rm red}}(u)=\oint_{\Gamma_0}{\rm d}v\,\Delta^\prime_{{\rm red}}(v)
K(v,u)
\end{equation}
and write the corresponding dispersion relation we find
\begin{equation}
{\cal D}\Delta_{{\rm red}}=2\sum_{N=1}^\infty\,j_{{\rm red}}^{[\epsilon]\prime}
\ \check\star\ (K^{[2N]}-K^{[-2N]}).
\end{equation}
Here the left hand side is the contribution of the narrow strip only 
(the pole terms vanish) and the right hand side is simply the sum of 
contributions of the integrals along the even cuts.  Using the method
explained in section~5 we can \lq\lq integrate" this relation and get
\begin{equation}
\Delta_{{\rm red}}=2\sum_{N=1}^\infty\,j_{{\rm red}}^{[\epsilon]}
\ \check\star\ (K^{[2N]}-K^{[-2N]}).
\end{equation}

\subsection{Determination of $\Delta_R$}

The dispersion relation for $\Delta_R$ can be written down using 
(\ref{D12RL}) and (\ref{disc12Rpm}). Proceeding as before we have
\begin{equation}
\begin{split}
\Gamma_R(u)=\oint_{\Gamma_0}{\rm d}v\,\Delta^\prime_R(v)&K(v,u)=
({\cal D}\Delta_R)(u)
+\oint_{[\gamma,2,\infty]}{\rm d}v\,
[\ln^\prime T_{1,1}^+(v)-\ln^\prime {\cal F}^+(v)]K(v,u)\\
&+\oint_{[-\infty,-2,-\gamma]}{\rm d}v\,
[\ln^\prime T_{1,1}^+(v)-\ln^\prime {\cal F}^+(v)]K(v,u).
\label{GammaR}
\end{split}
\end{equation}
The alternative calculation uses the explicit form of $D_{12R}^{(\pm2N)}$
and its direct integration along the cuts. The contribution of the upper
cuts is
\begin{equation}
\begin{split}
\Gamma^{{\rm upper}}_R(u)&=\sum_{N=1}^\infty\,\int \hspace{-3.9mm} \square
\,{\rm d}v\,K^{[2N]}(v,u)D^{(2N)\prime}_{12R}(v)\\
=&-\int_{-\infty}^\infty{\rm d}v\,K^{[\gamma]}(v,u)
\Lambda_-^{[\gamma]\prime}(v)
+\oint_{[\gamma,2,\infty]}{\rm d}v\,K(v,u)\Lambda_-^\prime(v)\\
&-\sum_{m=1}^\infty\int_{-\infty}^\infty{\rm d}v\,K^{[m+\gamma]}(v,u)
\Lambda_m^{[\gamma]\prime}(v)
+\sum_{m=1}^\infty
\oint_{[\gamma,m,\infty]}{\rm d}v\,K^{[m]}(v,u)\Lambda_m^\prime(v).
\end{split}
\end{equation}
Let us consider now the $\Lambda_m$ pole terms ($\oint\Lambda^\prime_m$ terms)
separately:
\begin{equation}
\begin{split}
&\sum_{m=1}^\infty\oint_{[\gamma+1,m+1,\infty]}{\rm d}v\,
K^{[m-1]}(v,u)\ln^\prime T_{m+1,1}(v)\\
+&\sum_{m=1}^\infty\oint_{[\gamma-1,m-1,\infty]}{\rm d}v\,
K^{[m+1]}(v,u)\ln^\prime T_{m+1,1}(v)\\
-&\sum_{m=0}^\infty\oint_{[\gamma,m+1,\infty]}{\rm d}v\,
K^{[m+1]}(v,u)\ln^\prime T_{m+1,1}(v)\\
-&\sum_{m=2}^\infty\oint_{[\gamma,m-1,\infty]}{\rm d}v\,
K^{[m-1]}(v,u)\ln^\prime T_{m+1,1}(v)
\end{split}
\end{equation}
We first note that in the integration contours $m-1$ can be changed
to $m+1$. This is possible because $T_{m,1}$ has no 
zeroes/poles/discontinuities on the $m-2$ cut for $m=3,4,\dots$ and
$T_{2,1}$ has no poles/discontinuities on the real cut while the
contribution of its real zeroes, as we have seen, has to be omitted.
We can also change all integrals to have contours of the type
$[\gamma,m+1,\infty]$ but here the change of $\gamma\pm1$ to $\gamma$
requires to add to this sum the corrections
\begin{equation}
%\begin{split}
-\sum_{m=1}^\infty\oint_{[\gamma,\gamma+1]}{\rm d}v\,
K^{[m-1]}(v,u)\ln^\prime T_{m+1,1}(v)\\
+\sum_{m=1}^\infty\oint_{[\gamma-1,\gamma]}{\rm d}v\,
K^{[m+1]}(v,u)\ln^\prime T_{m+1,1}(v).
%\end{split}
\end{equation}
The rest of the sum (after taking into account that most terms cancel)
simplifies to:
\begin{equation}
%\begin{split}
\oint_{[\gamma,2,\infty]}{\rm d}v\,K(v,u)\ln^\prime T_{2,1}(v)
-\oint_{[\gamma,2,\infty]}{\rm d}v\,K(v,u)\ln^\prime T_{1,1}^-(v)
+\oint_{[\gamma-1,\gamma]}{\rm d}v\,K^+(v,u)\ln^\prime T_{1,1}(v).
%\end{split}
\end{equation}
Adding also the pole terms corresponding to $\Lambda_-$
\begin{equation}
\oint_{[\gamma,2,\infty]}{\rm d}v\,K(v,u)\left[\ln^\prime T^+_{1,1}(v)
+\ln^\prime T^-_{1,1}(v)-\ln^\prime T_{2,1}(v)\right]
\end{equation}
the sum of all pole terms becomes:
\begin{equation}
\begin{split}
&-\sum_{m=1}^\infty\oint_{[\gamma,\gamma+1]}{\rm d}v\,
K^{[m-1]}(v,u)\ln^\prime T_{m+1,1}(v)\\
&+\sum_{m=0}^\infty\oint_{[\gamma-1,\gamma]}{\rm d}v\,
K^{[m+1]}(v,u)\ln^\prime T_{m+1,1}(v)
+\oint_{[\gamma,2,\infty]}{\rm d}v\,
K(v,u)\ln^\prime T^+_{1,1}(v).
\end{split}
\end{equation}
This can be simplified further using the relation $T_{m,1}=(-1)^{m-1}
\tau_m\sigma_m$ and the facts that $\sigma_m$ has no zeroes/poles near the
physical strip and $\tau_1^+$ has no zeroes/poles on the even cuts:
\begin{equation}
\begin{split}
-&\sum_{m=2}^\infty\oint_{[\gamma,\gamma+1]}{\rm d}v\,K^{[m-2]}(v,u)
\ln^\prime\tau_m(v)
+\sum_{m=1}^\infty\oint_{[\gamma-1,\gamma]}{\rm d}v\,K^{[m]}(v,u)
\ln^\prime\tau_m(v)\\
+&\int_{-\infty}^\infty{\rm d}v\,K^{[\gamma]}(v,u)
\ln^\prime\tau_1^{[1+\gamma]}(v)
+\oint_{[\gamma,2,\infty]}{\rm d}v\,
K(v,u)\ln^\prime \sigma^+_1(v).
\end{split}
\end{equation}
It remains to calculate the $\int_{-\infty}^\infty$ parts. We write these
contributions using the combinations (already used in section~4 for the
construction of the T-system elements)
\begin{equation}
{\mathscr L}_\pm=\ln\left[-\tau_2\left(1-\frac{1}{Y_\pm}\right)\right],\qquad
{\mathscr L}_m=\ln\left[\tau_m\tau_{m+2}
\left(1+\frac{1}{Y_{m\vert vw}}\right)\right]
\end{equation}
and find
\begin{equation}
\begin{split}
-&\int_{-\infty}^\infty{\rm d}v\,
K^{[\gamma]}(v,u)\Lambda_-^{[\gamma]\prime}(v)
-\sum_{m=1}^\infty\int_{-\infty}^\infty{\rm d}v\,
K^{[m+\gamma]}(v,u)\Lambda_m^{[\gamma]\prime}(v)\\
=-&\int_{-\infty}^\infty{\rm d}v\,
K^{[\gamma]}(v,u){\mathscr L}_-^{[\gamma]\prime}(v)
-\sum_{m=1}^\infty\int_{-\infty}^\infty{\rm d}v\,
K^{[m+\gamma]}(v,u){\mathscr L}_m^{[\gamma]\prime}(v)\\
+&\int_{-\infty}^\infty{\rm d}v\,
K^{[\gamma]}(v,u)\ln^\prime\tau_2^{[\gamma]}(v)
+\sum_{m=1}^\infty\int_{-\infty}^\infty{\rm d}v\,
K^{[m+\gamma]}(v,u)\left[\ln^\prime\tau_m^{[\gamma]}(v)
+\ln^\prime\tau_{m+2}^{[\gamma]}(v)\right].
\end{split}
\end{equation}
Adding everything together and using the identity $\tau_m^+\tau_m^-\equiv1$
in the form 
$\ln^\prime\tau_m^{[\gamma-1]}+\ln^\prime\tau_m^{[\gamma+1]}\equiv0$
we finally have
\begin{equation}
\begin{split}
\Gamma^{{\rm upper}}_R(u)&=\oint_{[\gamma,2,\infty]}{\rm d}v\,
K(v,u)\ln^\prime\sigma_1^+(v)\\
&-\int_{-\infty}^\infty{\rm d}v\,K^{[\epsilon]}(v,u)
{\mathscr L}_-^{[\epsilon]\prime}(v)
-\sum_{m=1}^\infty\int_{-\infty}^\infty{\rm d}v\,K^{[m]}(v,u)
{\mathscr L}_m^\prime(v).
\label{GammaRup}
\end{split}
\end{equation}
Similarly for the contribution of the lower half plane cuts we have
\begin{equation}
\begin{split}
\Gamma^{{\rm lower}}_R(u)&=\oint_{[-\infty,-2,-\gamma]}{\rm d}v\,
K(v,u)\left[\ln^\prime\sigma_1^+(v)
-\ln^\prime{\cal F}^+(v)-\ln^\prime{\cal G}^-(v)\right]\\
&-\int_{-\infty}^\infty{\rm d}v\,K^{[-\epsilon]}(v,u)
{\mathscr L}_+^{[-\epsilon]\prime}(v)
-\sum_{m=1}^\infty\int_{-\infty}^\infty{\rm d}v\,K^{[-m]}(v,u)
{\mathscr L}_m^\prime(v).
\label{GammaRlow}
\end{split}
\end{equation}

\subsection{The XXX gauge}

To calculate $\Delta_R$ we need to fix the gauge completely.
We will call this complete gauge fixing the XXX gauge and it will not be
our final gauge choice yet. Later we will have to perform an additional gauge 
transformation to arrive at the gauge in which all the T-functions are smooth 
deformation of the asymptotic solution. This \lq\lq intermediate" gauge,
which will be used in this subsection,
we call the XXX gauge because in the $g\rightarrow0$ limit the system
of functions $Y_{m\vert vw}$, $T_{m,1}$ decouples from the rest and they form
the Y-system and T-system of the XXX spin model (the latter in a gauge most 
natural in that model, namely in which the $T_{m,1}$ functions are polynomials
in the spectral parameter $u$). 

The XXX gauge is fixed by adding the requirements (in addition to those
already imposed in section~4 and this section):
\begin{itemize} 

\item ${\cal F}_{{\rm XXX}}^+$: no zeroes/poles in the upper 
half plane (no zeroes/poles on the real line) except poles at positions $u_j^+$
($j=1,2,\dots,N$).

\item ${\cal G}_{{\rm XXX}}^-$: no zeroes/poles in the lower 
half plane.

\end{itemize} 

Recalling that $T_{1,1}^{{\rm XXX}}=\tau_1\sigma_1$ we can express 
${\cal D}\Delta_R$ comparing (\ref{GammaR}) to the sum of
(\ref{GammaRup}) and (\ref{GammaRlow}). We find 
\begin{equation}
\begin{split}
{\cal D}&\Delta_R(u)=-\int_{-\infty}^\infty{\rm d}v\,
{\mathscr L}_-^{[\gamma]\prime}(v)K^{[\gamma]}(v,u)
-\int_{-\infty}^\infty{\rm d}v\,
{\mathscr L}_+^{[-\epsilon]\prime}(v)K^{[-\epsilon]}(v,u)\\
&-\sum_{m=1}^\infty\int_{-\infty}^\infty{\rm d}v\,
{\mathscr L}^\prime_m(v)k_m(v,u)+\oint_{[\gamma,2,\infty]}{\rm d}v\,\left[
\ln^\prime{\cal F}^+(v)-\ln^\prime\tau_1^+(v)\right]K(v,u)\\
&\qquad\qquad +\oint_{[-\infty,-2,-\gamma]}{\rm d}v\,
K(v,u)[-\ln^\prime\tau_1^+(v)].
\label{GammaRres}
\end{split}
\end{equation}
We can calculate the pole terms ($\oint$ terms) of this expression using
the residue theorem:
\begin{equation}
-2\pi i\sum_{j=1}^NK(u_j^+,u)+2\pi i\sum_{j=1}^N\sum_{\nu=-\infty}^\infty
\left\{K(u_j^++\frac{4\nu i}{g},u)-K(u_j^-+\frac{4\nu i}{g},u)\right\}.
\end{equation}
Their contribution, after \lq\lq integration", as explained in section~5,
becomes
\begin{equation}
{\cal W}(u)=\sum_{j=1}^N\sigma(u,u_j^+)
+\sum_{j=1}^N\sum_{\nu=-\infty}^\infty\left\{
\sigma(u,u_j^-+\frac{4\nu i}{g})-\sigma(u,,u_j^++\frac{4\nu i}{g})\right\}.
\end{equation}
Note that using the definition
\begin{equation}
\vartheta_1^+(u)=\prod_{j=1}^N\prod_{\nu=-\infty}^\infty\frac
{S(u,u_j^-+\frac{4\nu i}{g})}{S(u,u_j^++\frac{4\nu i}{g})},
\end{equation}
where the notation indicates that this function has exactly the same
zeroes/poles as $\tau_1^+$, we have
\begin{equation}
{\rm e}^{{\cal W}(u)}=\vartheta_1^+(u)\prod_{j=1}^NS(u,u_j^+).
\end{equation}
We can now write the \lq\lq integrated" version of (\ref{GammaRres}):
\begin{equation}
\begin{split}
\Delta_R(u)=-\int_{-\infty}^\infty{\rm d}v\,&{\mathscr L}_-^{[\gamma]}(v)
K^{[\gamma]}(v,u)
-\int_{-\infty}^\infty{\rm d}v\,{\mathscr L}_+^{[-\epsilon]}(v)
K^{[-\epsilon]}(v,u)\\
-&\sum_{m=1}^\infty\int_{-\infty}^\infty{\rm d}v\,
{\mathscr L}_m(v)k_m(v,u)+{\cal W}(u)-\ln x^2(u).
\label{DeltaRres0}
\end{split}
\end{equation}
Note that this formula is valid just above the real line in the strip 
$0<{\rm Im}u<\frac{\gamma}{g}$.

The last term in (\ref{DeltaRres0}) is necessary to balance the large
$\vert u\vert$ asymptotics of the equation. We know that in this limit
(just above the real line)
\begin{equation}
{\mathscr L}_+(u),\,{\mathscr L}_-(u)\approx-\ln\vert u\vert,\qquad
\Delta_R(u)\approx\ln\vert u\vert
\end{equation}
and we see that (\ref{DeltaRres0}) is asymptotically correct because
if a function $f$ behaves asymptotically as
$f(u)\approx\ln\vert u\vert$ then convolution with the kernel $K^{[\alpha]}$
gives
\begin{equation}
f\star K^{[\alpha]}\approx-\frac{1}{2}\ln\vert u\vert.
\end{equation}

Finally by manipulating the integrals containing 
${\mathscr L}_+,\,{\mathscr L}_-$ we write our final result for the 
discontinuity $\Delta_R$:
\begin{equation}
\begin{split}
\Delta_R(u)={\mathscr L}_-(u)-&\int_{-2}^2{\rm d}v\,
[{\mathscr L}_-(v)+{\mathscr L}_+(v)]K(v,u)\\
-&\sum_{m=1}^\infty\int_{-\infty}^\infty{\rm d}v\,
{\mathscr L}_m(v)k_m(v,u)+{\cal W}(u)-\ln x^2(u).
\label{DeltaRres}
\end{split}
\end{equation}
Note that the last term is chosen here so that $\Delta_R(\pm2)=0$ is
satisfied. The price we have to pay is that this term creates a cut
along the imaginary axis (but neither $\Delta^\prime_R(u)$ nor
${\rm e}^{\Delta_R(u)}$ have discontinuities there).

Our final result for the discontinuity $\Delta(u)$ in the ${\alg{sl}(2)}$
(sub-)sector is
\begin{equation}
\begin{split}
&\qquad\qquad\Delta=2\Delta_R+\Delta_d+\Delta_{{\rm red}}\\
&=2{\mathscr L}_--2({\mathscr L}_-+{\mathscr L}_+)\ \hat\star\ K-
2\sum_{m=1}^\infty{\mathscr L}_m\star k_m+
2{\cal W}-L\ln x^2+\ln\frac{{\cal D}_1^+}{({\cal D}_1^+)_*}+\Delta_{{\rm red}}.
%\sum_{Q=1}^\infty L_Q\star\Sigma_Q
\end{split}
\label{Deltares}
\end{equation}
Here we have used (\ref{yd}) to write
\begin{equation}
\Delta_d=-J\ln x^2+\ln\frac{{\cal D}_1^+}{({\cal D}_1^+)_*}.
\end{equation}
We note that the renormalization $J\rightarrow L=J+2$ is due to the addition
of the zero mode contribution in (\ref{DeltaRres0}) and seems to be universal
(at least for the case of states in the ${\alg{sl}(2)}$ (sub-)sector).

The result (\ref{Deltares}), together with $J^{(\alpha)}$ calculated in 
section~5, completes the set of TBA integral equations of section~3 for the
excited states in this sector of the model. This system of integral equations
is now closed. It still has to be supplemented by the quantization
conditions for the discrete parameters appearing in the source terms. This
will be discussed in section~9.

In this section we obtained the result (\ref{DeltaRres}) by a long direct
calculation. An alternative logic could have been to simply postulate
the result (\ref{DeltaRres}) for $p(u)=\Delta_R(u)$ and show that the 
requirements on the upper/lower half plane behaviour of the 
${\cal F}^+$/${\cal G}^-$ functions, which we used in the calculation, 
are indeed satisfied.

To show this, we start from
\begin{equation}
T^{{\rm XXX}}_{1,1}=\tau_1\sigma_1,\qquad\quad \sigma_1=\frac{q^+}{q^-}
\sigma_1^{(0)},
\end{equation}
where
\begin{equation}
\sigma_1^{(0)}=\exp\left\{{\mathscr L}_-^{[\epsilon]}\star(\kappa^--\kappa^+)
+\sum_{m=1}^\infty{\mathscr L}_m\star(\kappa^{[-m-1]}-\kappa^{[m+1]})
\right\}.
\end{equation}
Here we introduced the notation
\begin{equation}
\kappa(v,u)=\frac{1}{2\pi i}\,\frac{1}{v-u},\qquad\qquad
K_a=\kappa^{[-a]}-\kappa^{[a]}.
\end{equation}
Note that $K(v,u)-\kappa(v,u)$ is regular at $v=u$.

The discontinuity relation is
\begin{equation}
\frac{q(u+i\epsilon)}{q(u-i\epsilon)}={\rm e}^{-p(u+i\epsilon)},\qquad
\vert u\vert\geq2
\end{equation}
and just above the real line, in the strip $0<{\rm Im}u<\frac{\gamma}{g}$
we have
\begin{equation}
p={\mathscr L}_--({\mathscr L}_-+{\mathscr L}_+)\ \hat\star\ K-
\sum_{m=1}^\infty{\mathscr L}_m\star k_m+{\cal W}-\ln x^2
\end{equation}
and
\begin{equation}
\sigma_1^{(0)+}=\exp\left\{{\mathscr L}_-+{\mathscr L}_-^{[\epsilon]}\star
(\kappa^{--}-\kappa)+\sum_{m=1}^\infty{\mathscr L}_m\star(\kappa^{[-m-2]}
-\kappa^{[m]})\right\}
\end{equation}
and finally
\begin{equation}
\begin{split}
{\cal F}^+_{{\rm XXX}}&=\left(T_{1,1}^{{\rm XXX}}\right)^+{\rm e}^{-p}=
x^2\frac{q^{++}}{q}\,\frac{\tau_1^+}{{\rm e}^{\cal W}}\,\exp\Big\{
({\mathscr L}_-+{\mathscr L}_+)\ \hat\star\ K\\
+&{\mathscr L}_-^{[\epsilon]}\star(\kappa^{--}-\kappa)
+\sum_{m=1}^\infty{\mathscr L}_m\star(K^{[m]}-\kappa^{[m]}+
K^{[-m]}+\kappa^{[-m-2]})\Big\}.
\end{split}
\end{equation}
From this result we see that there are indeed no zeroes/poles/discontinuities
in the upper half plane, except for the poles at the positions $u_j^+$.

Similarly, just below the real line, in the strip 
$-\frac{\gamma}{g}<{\rm Im}u<0$ we have
\begin{equation}
\sigma_1^{(0)-}=\exp\left\{{\mathscr L}_-+{\mathscr L}_-^{[\epsilon]}\star
(\kappa-\kappa^{++})+\sum_{m=1}^\infty{\mathscr L}_m\star(\kappa^{[-m]}
-\kappa^{[m+2]})\right\},
\end{equation}
\begin{equation}
p=-{\mathscr L}_+-({\mathscr L}_-+{\mathscr L}_+)\ \hat\star\ K-
\sum_{m=1}^\infty{\mathscr L}_m\star k_m+{\cal W}-\ln x^2,
\end{equation}
and noting that from (\ref{Yvw1cut}) we have $I={\mathscr L}_--
{\mathscr L}_+$
\begin{equation}
m=I-p={\mathscr L}_-+({\mathscr L}_-+{\mathscr L}_+)\ \hat\star\ K+
\sum_{m=1}^\infty{\mathscr L}_m\star k_m-{\cal W}+\ln x^2,
\end{equation}
and finally
\begin{equation}
\begin{split}
{\cal G}^-_{{\rm XXX}}&=\left(T_{1,1}^{{\rm XXX}}\right)^-
{\rm e}^{-m}=\frac{1}{x^2}\,
\frac{q}{q^{--}}\,\frac{{\rm e}^{\cal W}}{\tau_1^+}\,\exp\Big\{
-({\mathscr L}_-+{\mathscr L}_+)\ \hat\star\ K\\
+&{\mathscr L}_-^{[\epsilon]}\star(\kappa-\kappa^{++})
+\sum_{m=1}^\infty{\mathscr L}_m\star(\kappa^{[-m]}-K^{[-m]}-
K^{[m]}-\kappa^{[m+2]})\Big\}.
\end{split}
\end{equation}
We see that there are indeed no zeroes/poles/discontinuities
in this expression in the lower half plane.

\subsection{Complete gauge fixing}

It is possible to show that the XXX gauge we have been using in this
section is a complete gauge fixing. This means that given an exact solution
of the Y-system equations, which also satisfies the reality conditions and
the relation between $Y_-$ and $Y_+$ and has the cut structure described
in section~2, we can always construct the corresponding XXX gauge T-system
elements $T^{{\rm XXX}}_{a,s}$, which satisfy all the requirements
listed below and this construction is unique.

The requirements are
\begin{itemize} 

\item $T^{{\rm XXX}}_{0,s}\equiv1$.

\item $T^{{\rm XXX}}_{a,0}$ are given as constructed explicitly in section~4
using the chain lemma.

\item $T^{{\rm XXX}}_{a,1}$ have discontinuities along the cuts 
$\pm(a+2m)$, $m=0,1,\dots$

\item The roots of $T^{{\rm XXX}}_{a,1}$ in the physical strip are the same 
as those of $\tau_a$ and there are no poles in this strip.

\item ${\cal F}_{{\rm XXX}}^+$: no zeroes/poles/discontinuities in the upper 
half plane (no zeroes/poles on the real line) except poles at positions $u_j^+$
($j=1,2,\dots,N$).

\item ${\cal G}_{{\rm XXX}}^-$: no zeroes/poles/discontinuities in the lower 
half plane.

\item The large $\vert u\vert$ behaviour is the same as for the asymptotic
solution.

\end{itemize} 

We now perform the final gauge transformation which brings the T-system
solution in a gauge (we will call it the BA gauge) where the T-system
functions $T_{a,s}$ for $s\geq0$ are close to the asymptotic (Bethe Ansatz)
solution $T_{a,s}^{(0)}$. This is achieved by defining
\begin{equation}
T_{1,1}=\beta\,T^{{\rm XXX}}_{1,1},\qquad\quad
\beta=\frac{Q^{--}}{Q}.
\label{BAbeta}
\end{equation}
We see that $T_{1,1}$ has no zeroes/poles in the physical strip.
From
\begin{equation}
{\cal F}^+=\frac{Q^-}{Q^+}\,{\cal F}^+_{{\rm XXX}},\qquad\quad
{\cal G}^-=\frac{Q^{[-3]}}{Q^-}\,{\cal G}^-_{{\rm XXX}}
\end{equation}
we see that ${\cal F}^+$/${\cal G}^-$ has no zeroes/poles/discontinuities
in the upper/lower half plane. 

From the list of requirements above and the modification induced by
(\ref{BAbeta}) we see that the BA gauge T-functions are indeed
smooth deformations of the asymptotic solution, satisfying the same
requirements. Note that the final results for $p=\Delta_R$ and the full 
$\Delta$ are unchanged since the transformation (\ref{BAbeta}) is meromorphic.



==> nzintro <==


An important problem in the AdS/CFT correspondence \cite{adscft} is the calculation of
anomalous dimensions in the planar ${\cal {N}}=4$ super Yang-Mills theory (SYM)
or equivalently the energies of the dual $AdS_5 \times S^5$ string sigma-model.

The integrability discovered on both sides of the correspondence provided us with
an efficient mathematical apparatus to compute the exact spectrum of the planar
AdS/CFT models. As the central object of integrability the 2-particle S-matrix of the
model \cite{S,dressing,dresscross} plays a prominent {role}{\footnote{For a recent review see \cite{S1,S2} and
references therein.}} and is indispensable for the methods which enable us to compute the exact spectrum.

First, the spectrum of long operators or equivalently states with large R-charge
$J$ was determined by the asymptotic Bethe Ansatz (ABA) \cite{BS,S1}, which describes 
all polynomial corrections in $1/J$. 

Later, the leading exponentially small {corrections}{\footnote{These are the so 
called wrapping corrections.}} in $J$ could be taken into account by means of
the generalized L\"uscher formulae \cite{Luscher85,JL07,BJ08}. For the Konishi field their small coupling
expansion led to beautiful agreement with direct 4-loop field theoretical computations \cite{Sieg,Vel}.
For a certain class of states in the ${\alg{sl}(2)}$ sector the 4- and 5-loop expansion of these formulae 
\cite{Bajnok:2008qj,BJ09,Lukowski:2009ce} also satisfy
nontrivial consistency checks dictated by perturbation theory considerations in the
planar ${\cal {N}}=4$ SYM \cite{KL02,40_5}.

The exact energies, which resum all wrapping corrections in $J$, can be obtained by
the application of the Thermodynamic Bethe Ansatz method \cite{Zami} to the doubly
Wick rotated $AdS_5 \times S^5$ string sigma-model called the mirror model \cite{AJK,AF07}.

Strictly speaking the TBA method provides only the ground state energy of the model in finite
volume and its extension to excited states is only a conjecture even if
in most of the cases it rests on solid grounds. Based on the corresponding 
string-hypothesis \cite{AF09a} the ground state TBA equations of the $AdS_5 \times S^5$
mirror model were constructed in \cite{Bombardelli:2009ns,GKKV09,AF09b}
and simplified in \cite{AF09d}.
In AdS/CFT the ground state TBA equations do not give much information about the
spectrum since the ground state is protected by supersymmetry, i.e. $E_0(L)=0$.

The ground state equations are important nevertheless because they serve as
starting point for the excited state equations. An important further discovery is that
the Y-{functions}{\footnote{I.e. unknown functions of the TBA equations}} of the
mirror TBA equations satisfy the so called Y-system functional equations \cite{GKV09}.
The Y-functions can be rephrased in the language of T-functions  satisfying
the so-called T-system. The T-system of AdS/CFT lives on a T-hook \cite{GKV09}.
The discovery of the Y- and T-systems (see Figs. 1, 2) made it possible to determine the asymptotic
(large $J$) solutions of the excited state TBA problem. The asymptotic solution
is constructed so that the ABA and the generalized L\"uscher formulae are reproduced. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[htbp]
%\begin{center}
%\begin{picture}(280,60)  \epsfxsize=70mm
%\put(-70,-55) {\epsfbox{Yads.eps}}
%\put(145,-55) {\epsfbox{Tads.eps}}
%\put(-75,-70) {\parbox{140mm}
%{\caption{ \label{6f}\protect {\footnotesize
% The domain of definition for the Y-system (on the left) and for the T-system (on the right). }}}}
%\end{picture}
%\end{center}
%\vspace{2.3cm}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Based on previously elaborated examples in lattice models \cite{KPS,33B} and in relativistic quantum field theory (QFT)
\cite{DT,BLZ,BH-SG,BH34}, the common experience is that excited state TBA equations differ from
the ground state ones only in source {terms}
%{\footnote{Source term: such term in the TBA equations,which are not convolutions of a kernel and a function of some Y-function.}} 
and in quantization conditions imposed on objects appearing in the arguments of these terms.
These source terms can be found by various methods like analytical continuation
in some parameter of the model  \cite{DT}, deforming the integration contour of the ground
state equations \cite{KPS,Arutyunov:2009ax} or transforming the Y-system functional relations to integral 
equations \cite{KPS,33B,BH-SG,BH34}.
In AdS/CFT the analytical continuation \cite{GKKV09,GKV09b} and contour deformation \cite{Arutyunov:2009ax} 
methods together with requiring consistency with the large $J$ asymptotic solution were successfully applied 
to find the excited state TBA equations for certain states of the ${\alg{sl}(2)}$ sector of the model.

Since the TBA equations in AdS/CFT still cannot be derived from first principles it is
important to test them carefully. In the strong coupling limit it was shown  \cite{Gromov,ujKazi} 
that the TBA equations reproduce the 1-loop string energies in the semi-classical limit and
the strong coupling expansion of the energy of the Konishi state fitted from numerical TBA
computations  \cite{GKV09b,Frolnum} was found to be consistent with direct string theory computations \cite{StrongKonishi}.
At weak coupling 5-loop TBA results for the twist-2 states 
agree \cite{AFS,BHxxx,BH-BJ} with those based on the generalized  L\"uscher formula.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In integrable relativistic QFTs the Y-system equations supplemented by some analyticity
%properties of the Y-functions was an efficient tool to derive excited state TBA equations.
%However, until the appearance of ref. \cite{Tateo1} this method failed to work in AdS/CFT since
%here the Y-functions are not meromorphic functions like in the relativistic cases, but 
%have nontrivial branch cut structure. The main discovery of ref. \cite{Tateo1} is that
%the Y-system functional equation can be supplemented by state independent discontinuity
%relations for the square-root branch cuts of the Y-functions. These two sets of functional 
%equations plus some analyticity assumption on the distribution of zeroes and poles of the 
%Y-functions are enough to transform the Y-system to TBA equations. In this spirit the ground
%state TBA equations were derived \cite{Tateo1} assuming that none of the Y-functions have {local}{
%\footnote{Here the word "local" means zeros or poles.}} singularities on the entire complex plane.
 
% In this paper extend the method to excited states as well. 
% The discontinuity relations discovered in \cite{Tateo1} were based on the ground state equations and
% were claimed to be valid for excited states as well.
% Here we show that for excited states the asymptotic solutions of the Y-system non-trivially
% satisfy these relations.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Though the analytical continuation and contour deformation methods provide the TBA equations
for excited states it is important to derive the TBA equations from the Y-system functional relations
as well. The main advantage of the Y-system based method is that the infinite Y-system can be solved
via the T-system and the related T-Q relations, thus it opens the way towards the NLIE formulation
of the AdS/CFT spectral problem. 

However, until ref. \cite{Tateo1} appeared, the Y-system based derivation of the TBA equations 
was impossible because the Y-functions are not meromorphic functions like in the relativistic models and
have nontrivial discontinuity structure.
The main discovery of ref.~\cite{Tateo1} was that this extra difficulty can be overcome for the 
ground state if the Y-system equations are supplemented by appropriate functional relations for
the square-root discontinuities of the Y-functions. The Y-system equations supplemented by the discontinuity functional
relations plus some analiticity assumption on the distribution of zeroes and poles of the Y-functions
are sufficient to transform the Y-system to TBA integral equations. 
In this spirit the ground state TBA equations (including the dressing kernel)
were derived \cite{Tateo1} assuming that none of the Y-functions have 
{local}{\footnote{Here the word \lq\lq local" means zeroes or poles.}} singularities in the entire complex plane.

It was conjectured in ref. \cite{Tateo1} that the  form of the discontinuity functional relations is 
state independent. If true, this allows us to derive excited state TBA equations from the 
Y-system as well. In this paper we carry out the Y-system based derivation of the excited state TBA equations.
As a first step we have checked that the conjecture is true in the asymptotic limit
and found that the asymptotic solutions given in appendix C satisfy the discontinuity relations
nontrivially.

Furthermore we  show that we do not need to  know the \lq\lq local" analyticity properties of the Y-functions
in the entire complex plane, it is sufficient to know their behaviour in certain regions near the real line.
This means that the assumption of ref. \cite{Tateo1} concerning the \lq\lq local" singularities of the 
ground state Y-functions is too restricting and can be weakened. Indeed, in \cite{Tateo2}   
it has been shown numerically that the ground state Y-functions do have local singularities in the
complex plane, but they lie too far from the real line to modify the form of the equations \cite{Tateo3}. 
 
Throughout the paper we assume that within certain regions of the complex plane the excited state
Y-functions are smooth deformations of the asymptotic solution given in \cite{GKV09}.
More precisely, we only discuss that part of the parameter space where the exact solution has
(qualitatively) the same analytic properties as the corresponding asymptotic solution. In practice,
if the size of the system ($J$) together with other quantum numbers are fixed, this is realized for
small enough coupling $g$. For larger $g$ the TBA equations for the given state may undergo phase transitions
similarly to what was found in \cite{Frolnum}. In this paper we restrict our attention to the form
of the TBA equations valid in the vicinity of the asymptotic solution. 
Then assuming that the solution of the Y-system is found we construct the T-functions in an appropriate
gauge. These T-functions are also smooth deformations of their asymptotic forms.

The benefit of introducing the T-functions is 2-fold. On the one hand they serve as internal variables
in terms of which the discontinuity relations and the derivation of the TBA equations
simplifies drastically. On the other hand T-functions seem to be more fundamental objects from the
point of view of the AdS/CFT spectral problem. For example we show that the complicated TBA 
energy formula becomes a very simple expression containing the single T-function $T_{1,0}$.
No doubt this fact indicates that there is an integrable $psu(2,2|4)$ spin-chain in the background
such that the Hamiltonian is related to a transfer matrix of the model similarly to the cases of
lattice models and lattice regularizations \cite{devegasum} of integrable QFTs \cite{FR,LC} studied previuosly.

Our final equations agree with previous results of \cite{Arutyunov:2009ax}. 
%which have been tested successfully against
%weak \cite{} and strong coupling \cite{} results.
Our derivation is based on functional relations and analyticity assumptions which we know
are satisfied exactly in the asymptotic limit. Hence as a by-product our results prove analytically that the asymptotic solution 
satisfies the large $J$ limit of the TBA equations and also that the large $J$ limit of the exact Bethe
equations coincide with the ABA equations. This fact, although it 
played an important role in the extraction of the 5-loop L\"uscher terms from TBA \cite{AFS,BHxxx,BH-BJ},
has not been proven analytically so far. 

The organization of the paper is as follows. In the next section we introduce our starting relations
and assumptions. Section 3 contains important lemmas and the transformation of the Y-system to TBA integral
equations leaving the necessary discontinuities temporarily unspecified.
In section 4 we construct the T-system in a partially fixed special gauge 
which turns out to be very useful to simplify the derivation of the TBA equations. 
In section 5 and 6 we compute the so far undetermined discontinuities $Y_{-}^{(\alpha)}/Y_{+}^{(\alpha)}$
and $\Delta$ from dispersion relations and we fix completely our gauge choice for the T-functions.
In section 7 we derive the simplified version of the TBA equations, while section 8 contains their
canonical and hybrid form. In section 9 we discuss the quantization conditions and the
exact Bethe equations. Finally, in section 10 we discuss a simplified energy
formula. The paper is closed by our conclusions.
Appendix A contains the definitions of frequently used objects and kernels, appendix B the discussion of the branch cut 
discontinuities of the dressing part of the discontinuity function $\Delta$ and finally in appendix C 
the asymptotic solution of the Y- and T-system equations are presented. 





==> nzstart <==

Our starting point in this paper is the hypothesis that the same Y-system describes all excited
states in the planar AdS/CFT spectral problem \cite{GKV09}. The Y-system of AdS/CFT takes the standard form
\begin{equation} \label{Y}
Y_{a,s}^+ \, Y_{a,s}^-=\frac{(1+Y_{a,s-1}) \, (1+Y_{a,s+1})}{ (1+1/{Y_{a-1,s}}) \, (1+1/{Y_{a+1,s}})},    
\end{equation}  
but it lives on an $(a,s)$ lattice represented in Fig. 1. This is equivalent to imposing the
boundary conditions $Y_{0,s} \to \infty$, $Y_{2,|s|>2} \to \infty$ and $Y_{a>2,\pm 2} \to 0$ 
while the product $Y_{3,\pm 2} \, Y_{2,\pm 3}$ should be kept finite in order to $Y_{2,\pm 2}$ be finite. This
last requirement shows that the Y-system defined in the domain of Fig. 1
cannot form a closed set of equations because the new functions $Y_{3,\pm 2} \, Y_{2,\pm 3}$ enter 
the problem and we need additional equations (independent of the Y-system) to complete the system.

The Y-system is equivalent to a T-system defined on a T-hook of Fig. 2:
\begin{equation} \label{T}
T_{a,s}^+ \, T_{a,s}^-=T_{a+1,s} \, T_{a-1,s}+ T_{a,s+1} \, T_{a,s-1},
\end{equation}
where the relation to the $Y_{a,s}$ functions is given by
\begin{equation} \label{YT}
Y_{a,s}=\frac{T_{a,s+1} \, T_{a,s-1}}{T_{a+1,s} \, T_{a-1,s}}, \qquad 
1+Y_{a,s}=\frac{T_{a,s}^+ \, T_{a,s}^-}{T_{a+1,s} \, T_{a-1,s}}, \qquad
1+1/Y_{a,s}=\frac{T_{a,s}^+ \, T_{a,s}^-}{T_{a,s-1} \, T_{a,s+1}}.
\end{equation}
The T-equations can be extended to the infinite $(a,s)$ lattice by imposing the boundary conditions
that all $T_{a,s}=0$ outside the T-hook. The T-system is a more fundamental set of equations
than the Y-system because it forms a closed set of functional {equations}{\footnote{Here the word
\lq\lq closed" means that there are as many functional equations as T-functions.}} 
which determines all the Y-functions together with the supplementary combination 
$Y_{3,\pm 2} \, Y_{2,\pm 3}$.
The T-equations and the Y-functions given by (\ref{YT}) are invariant with respect to the 
gauge transformations
\begin{equation} \label{gauge0}
T_{a,s} \rightarrow g_1^{[a+s]} \, g_2^{[a-s]} \, g_3^{[s-a]} \, g_4^{[-s-a]} \, T_{a,s},
\end{equation}
with $g_{1,2,3,4}$ being arbitrary functions. In this paper we will choose a gauge where
$T_{0,s}=1$. This fixes $g_1 g_3=g_2 g_4=1$. 

It is known that in AdS/CFT the Y-functions have square root branch cuts and live on an 
infinite genus Riemann surface \cite{AF09b,AF09d,Tquant}. The different sheets of the Riemann surface
are connected through square-root branch cuts starting from the branch points with real parts $\pm 2$
and run to infinity along the lines with integer (in $1/g$ units) imaginary parts.
To avoid the complications connected to using different sheets we will use a convention where
all our functions are assumed to be defined on the first Riemann sheet, defined as the entire complex plane excluding the
above cuts. In our convention if we analytically continue a function through one of the cuts, this becomes a new function,
which can also be continued to the entire first Riemann sheet. We will often use the operation $f(u)\rightarrow f_*(u)$ corresponding to
analytic continuation of the function $f(u)$ through the real cut $\vert u\vert\geq2$. The construction of $f_*(u)$ consists of the two steps
of analytic continuation of $f(u)$ through the real cut followed by analytic extension of the new function to the entire first Riemann sheet.
Our functions are assumed to be meromorphic in the first Riemann sheet: they have discontinuities along some (but not necessarily all) 
of the cuts of the first Riemann sheet and cannot have other discontinuities but may have local singularities (zeroes and/or poles) 
in the sheet (and in some cases even on the cuts).  

Restricting the Y-functions to the first Riemann sheet
the Y-system equations supplemented by some analyticity information on the local singularities 
are not enough to derive the TBA integral equations. Some additional information on the discontinuities
is needed as well. According to the proposal of ref. \cite{Tateo1} this missing piece of information
is a set of functional equations relating the discontinuities in a state independent way. These discontinuity
equations translated to dispersion relations determine the extra $Y_{3,2} \, Y_{2,3}$ functions as well.

We will use the conventions of ref. \cite{Arutyunov:2009ax} throughout the paper. 
The Y-functions in these conventions are related to the $Y_{a,s}$ variables as follows:
\begin{equation}
Y_{-}^{(\alpha)}=-1/Y_{1,\alpha  1}, \qquad 
Y_{+}^{(\alpha)}=-Y_{2,\alpha  2}, \quad  \alpha=\pm \qquad Y_Q=Y_{Q,0} \quad  \quad Q=1,2,... \nonumber
\end{equation}
\begin{equation}
Y_{m|vw}^{(\alpha)}=1/Y_{m+1,\alpha 1} \qquad Y_{m|w}^{(\alpha)}=Y_{1,\alpha(m+1)} \qquad \alpha=\pm \quad %%@
m=1,2,...
\end{equation}
From the ground state equations we obtain the following structure for the locations of the branch cuts:
\begin{itemize}
\item $Y_{\pm}^{(\alpha)}(u): \qquad u+i \,2\, m/g \quad  \quad
m \in \mathbb{Z}$, 
\item $Y_m(u), \quad Y_{m|vw}^{(\alpha)}(u), \quad Y_{m|w}^{(\alpha)}(u): \qquad u\pm i \,(m+2 \,j)/g, \qquad
j=1,2,...,\infty $, 
\end{itemize}
where $u \in (-\infty,-2) \cup (2,\infty)$.
One of our main assumptions is that this structure remains valid for the excited states as well.
For later convenience we rewrite the discontinuity relations proposed in \cite{Tateo1} for the square-root branch cuts 
in the conventions we are using in this paper. They take the form
\begin{equation} \label{Y1cut}
\Delta=[\ln Y_1]_{+1},
\end{equation}
\begin{equation}   \label{Deltacut}
[\Delta]_{\pm 2N}= \pm \sum_{\alpha} \left(
\left[\ln \!  \left(1-\frac{1}{Y_{\mp}^{(\alpha)}}   \right)\right]_{\pm 2N}   \!
+\sum\limits_{m=1}^N \, \left[\ln  \! \left(1+\frac{1}{Y_{m|vw}^{(\alpha)}}\right)\right]_{\pm (2N-m)} 
\! \! \! \! \! \! \!  \!+ \! \ln \!  \left( \frac{Y_{-}^{(\alpha)}}{Y_{+}^{(\alpha)}} \right)  
\right)
\end{equation}
\begin{equation} \label{Ypmcut}
\left[ \ln \! \left( \frac{Y_{-}^{(\alpha)}}{Y_{+}^{(\alpha)}} \right) \right]_{\pm 2N}=
-\sum\limits_{Q=1}^N \, \left[ \ln \! \left( 1+Y_Q \right) \right]_{\pm (2N-Q)}
\end{equation}
with $N=1,2,...$ and
\begin{equation} \label{Yvw1cut}
\left[ \ln \! Y_{1|vw}^{(\alpha)} \right]_{\pm 1}=\ln \! 
\left( \frac{1-1/Y_{-}^{(\alpha)}}{1-1/Y_{+}^{(\alpha)}}   \right), \qquad
\left[ \ln \! Y_{1|w}^{(\alpha)} \right]_{\pm 1}=\ln \! 
\left( \frac{1-Y_{-}^{(\alpha)}}{1-Y_{+}^{(\alpha)}}   \right),
\end{equation}
where the symbol $[f]_Z$ with $Z \in \mathbb{Z}$ denotes the discontinuity of the function $f(u)$:
\begin{equation} \label{[f]_Z}
[f(u)]_Z=\lim_{\epsilon \to 0^+} \left( f(u+i \, Z/g+i \epsilon)- f(u+i \, Z/g-i \epsilon) \right), \qquad
u \in (-\infty,-2) \cup (2,\infty).
\end{equation}
In the sequel $[f(u)]_Z$ means the analytic extension of the discontinuity (\ref{[f]_Z}) to generic values
of $u$. Using the notation defined earlier in this section we can write 
$[f(u)]_Z=f^{[+Z]}(u)-(f^{[+Z]})_*(u)$ where $(f^{[+Z]})_*(u)$ is the 
{function}{\footnote{$f^{[\pm Z]}(u)=f(u \pm i \, Z/g)$, see appendix A.}}
obtained by analytical continuation of $(f^{[+Z]})(u)$ through the cut lying along the real line  
%$\mbox{Im} u=0$ %
and then extended to the first Riemann sheet.

Some important remarks on the interpretation of the discontinuity relations (\ref{Y1cut}-\ref{Yvw1cut})
are in order. As they stand, (\ref{Y1cut}-\ref{Yvw1cut}) are valid if the Y-function
combinations appearing in them have no logarithmic discontinuities crossing the lines of the square-root
discontinuities. In order to get rid of the difficulties caused by the logarithmic discontinuities we use
the derivative of the discontinuity relations (\ref{Y1cut}-\ref{Yvw1cut}) as our starting point and apply
dispersion relations for the derivatives of $\Delta$ and $\ln Y_{-}^{(\alpha)}/Y_{+}^{(\alpha)}$.
Then a second subtlety appears if there are local singularities of the Y-function combinations lying
exactly on the lines of square-root discontinuities. Such local singularities do not modify the discontinuity
relations, but they contribute to the corresponding dispersion relation through the residue theorem. To cure this problem
a finer interpretation of the discontinuity relations is necessary in which the contribution of such local
singularities are taken into account as well. 

To find the correct interpretation we can invoke the asymptotic solution. 
It can be shown that only (\ref{Deltacut}) at $N=1$ and at the positions of real poles 
of $1-1/Y_{\pm}^{(\alpha)}$ must be refined.
The term which causes the trouble is $\left[ \ln \left(1+{1}/{Y_{1|vw}^{(\alpha)}} 
\right)\right]_{\pm 1}$ on the right hand side of (\ref{Deltacut}), because its derivative has poles sitting right on the
{discontinuities}{\footnote {We note that other Y-combinations for other values of $N$ can also
have local singularities along the cuts under consideration, but they mutually cancel each other's
contribution. }} with $\mbox{Im} u=\pm 1/g$. This refined interpretation of (\ref{Y1cut}-\ref{Yvw1cut}) is necessary
only when they are translated to dispersion relations.
In order for the dispersion relation applied for the derivative of (\ref{Deltacut}) give the correct formula for 
$\Delta$ the following replacement must be done on the right hand side of (\ref{Deltacut}) at $N=1$:
\begin{equation} \label{CutInterpret}
\left[ \ln \left(1+\frac{1}{Y_{1|vw}^{(\alpha)}(u)} 
\right)\right]_{\pm 1} \rightarrow \left[ \ln \left \{ \left(1+\frac{1}{Y_{1|vw}^{(\alpha)}(u)} 
\right)  \frac{1}{p_2^\mp(u)} \right \}   \right]_{\pm 1},
\end{equation} 
where $p_2(u)$ is the polynomial having zeroes at the positions of the real zeroes 
of $Y_{\pm}^{(\alpha)}$ with absolute values larger than $2$.
In other words the poles corresponding to the zeroes of $p_2(u)$ must be ignored.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% there are no local log type branching 
%points of the Y-function combinations lying on the lines of discontinuities. Then in these isolated points
%of the square-branch cuts a finer interpretation of the discontinuity relations is necessary. 
%For the appropriate interpretation the asymptotic solution can be invoked. It can be shown that only in 
%(\ref{Deltacut}) at $N=1$ and at the positions of real poles of $1-1/Y_{\pm}^{(\alpha)}$ can be problems
% of interpretation.
%The term being responsible for this problem is $\left[ \ln \left(1+{1}/{Y_{1|vw}^{(\alpha)}} 
%\right)\right]_{\pm 1}$ on the right hand side, because it has log type branching points along the
%{cuts}{\footnote {We note that other $Y$-combinations for other values of $N$ can also
%have log type branching points along the cuts under consideration, but they mutually cancel each other's
%contribution. }} with $\mbox{Im} u=\pm 1$. The fine interpretation of  (\ref{Y1cut}-\ref{Yvw1cut}) is necessary
%when they are translated to dispersion relations.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In this paper we will use the derivative of the discontinuity relations so the log type branch cuts
%become poles. In the dispersion relations these points give nontrivial contributions through the residue
%theorem. In order for the dispersion relation derived from (\ref{Deltacut}) give the correct formula for 
%$\Delta$ the following replacement must be done on the right hand side of (\ref{Deltacut}) at $N=1$:
%\begin{equation} \label{CutInterpret}
%\left[ \ln \left(1+\frac{1}{Y_{1|vw}^{(\alpha)}(u)} 
%\right)\right]_{\pm 1} \rightarrow \left[ \ln \left \{ \left(1+\frac{1}{Y_{1|vw}^{(\alpha)}(u)} 
%\right)  p_2(u) \right \}   \right]_{\pm 1},
%\end{equation} 
%where $p_2(u)$ is the polynomial having zeroes at the positions of the real zeroes 
% of $1-1/Y_{\pm}^{(\alpha)}$ with absolute values larger than $2$.
%Though this modification does not influence the relations among the square-root discontinuities
%but it modifies the dispersion relation through the residue theorem. In other words the
%poles corresponding to the zeroes of $p_2(u)$ must be ignored.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We note that as a consequence of the definition (\ref{Y1cut}), and the fact that going around twice a square root branch point gives back
the original function, we have the relation 
\begin{equation} \label{Deltacut0}
\Delta(u)=-\Delta_*(u). 
\end{equation}

The Y-system (\ref{Y}) and the discontinuity relations (\ref{Y1cut}-\ref{Yvw1cut}) are not 
sufficient to derive the TBA equations. Some more information is needed about the discontinuities
lying along the real axis. 
Based on the properties of the solution for the ground state TBA equations and the similar properties of the
asymptotic solution for excited states, we require that the \lq\lq fermionic" Y-functions $Y^{(\alpha)}_\pm$
are analytic continuations of each other:
\begin{equation} \label{Y-cut0}
 Y_{-}^{(\alpha)}(u)=(Y_{+}^{(\alpha)})_*(u).
\end{equation}

We will also assume that all Y-functions are real analytic. This assumption
is based on the observations that the Y-functions are real analytic functions for the ground state
solution of the TBA equations and also in the asymptotic limit for excited state solutions. 
Since we consider the AdS/CFT Y-functions as smooth deformations
of their asymptotic counterparts we restrict ourselves to deformations that preserve the property
of real analyticity. We note that in the abcence of this assumption several TBA integral equations
could be set up (such that their asymptotic limit coincides). 

To summarize we assume that 
\begin{itemize}

\item Y-functions satisfy the Y-system equations (\ref{Y}). 

\item The discontinuities are related by the modified relations 
(\ref{Y1cut}-\ref{Yvw1cut}),(\ref{CutInterpret}).

\item $Y_{-}^{(\alpha)}(u)$ and $Y_{+}^{(\alpha)}(u)$
are related by (\ref{Y-cut0}).

\item The Y-functions are real analytic functions.

\item The Y-functions are smooth deformations of their asymptotic limit.

\end{itemize}

If one assumes that both $\Delta$ and $Y_{-}^{(\alpha)}/Y_{+}^{(\alpha)}$ are analytic and  
bounded near $\pm 2$ then their discontinuities must be zero at the branching points $\pm 2$. 
From this requirement and from (\ref{Deltacut0}), (\ref{Y-cut0}) it follows
that the combinations $\Delta(u)/\sqrt{4-u^2}$ and $\ln  (Y_{-}^{(\alpha)}/Y_{+}^{(\alpha)})/\sqrt{4-u^2}$ 
have no square root branch cuts along the real axis. These properties have been used in the derivation given
in ref. \cite{Tateo1} and we think it is important to emphasize them since they play very important
role also in our considerations.

The form of the discontinuity relations (\ref{Y1cut}-\ref{Yvw1cut}) and (\ref{Deltacut0}), (\ref{Y-cut0}) have 
been conjectured to be independent of the particular excited state of the $AdS_5 \times S^5$ sigma-model under consideration.
Using the formulae and results of appendices A, B, and C this conjecture can be proven to be valid for the asymptotic 
solutions. Here we will {verify}{\footnote{During the verification the upper case index $(\alpha)$
is ignored since in the limit under consideration the two wings of the Y-system become independent.
Furthermore we forget about possible logarithmic dicontinuities since (\ref{Y1cut}-\ref{Yvw1cut})
account for the contribution of the square-root discontinuities only. }}
the relations (\ref{Ypmcut}),(\ref{Yvw1cut}) and (\ref{Y-cut0}) in the asymptotic 
{limit}{\footnote{ Asymptotic limit: $J \to \infty$ or $g \to 0$.}}.
The (asymptotic) justification of (\ref{Deltacut}) will be presented in section 6.

With the help of the T-function representation of $Y_{-}^{(0)}/Y_{+}^{(0)}$ and the formulae
of appendix C it can be shown that asymptotically:
\begin{equation} \label{Ym/Yp(0)}
\ln \left( Y_{-}^{(0)}/Y_{+}^{(0)}\right)= \ln \frac{R_p \, B_m}{R_m \, B_p},
\end{equation}
from which $\left[\ln \left(Y_{-}^{(0)}/Y_{+}^{(0)}\right)\right]_{\pm 2N}=0$,
the asymptotic $(Y_Q \to 0)$ limit of (\ref{Ypmcut}), follows immediately.

The asymptotic verification of (\ref{Yvw1cut}) goes as follows. Using the T-representation:
\begin{equation} \label{Y1vw(0)cut}
\left[ \ln Y_{1|vw}^{(0)} \right]_{\pm 1}=-\left[ \ln Y_{2,1}^{(0)} \right]_{\pm 1}=
\left[ \ln \frac{T_{1,1}^{(0)}}{T_{2,2}^{(0)}} \right]_{\pm 1}.
\end{equation}
With the help of (\ref{T0sT0a0})-(\ref{G0}) it can be shown that:
\begin{equation} \label{T1122cut}
\left[ \ln \frac{T_{1,1}^{(0)}}{T_{2,2}^{(0)}} \right]_{\pm 1}=
\ln \frac{T_{1,1}^{(0)+} \, T_{1,1}^{(0)-}}{{\cal F}^{(0)+}  \, {\cal G}^{(0)-}} 
\frac{T_{2,3}^{(0)}}{T_{3,2}^{(0)}}=
\ln \frac{1+1/Y_{1,1}^{(0)}}{1+Y_{2,2}^{(0)}}=\ln \frac{1-Y_{-}^{(0)}}{1-Y_{+}^{(0)}}.
\end{equation}
Formulae (\ref{Y1vw(0)cut}) and (\ref{T1122cut}) together verify the first relation of 
(\ref{Yvw1cut}) while the
second relation follows from (\ref{T1122cut}) and the following two relations:
\begin{equation} \label{Y1w(0)cut}
\left[ \ln Y_{1|w}^{(0)} \right]_{\pm 1}=\left[ \ln Y_{1,2}^{(0)} \right]_{\pm 1}=
\left[ \ln \frac{T_{1,1}^{(0)}}{T_{2,2}^{(0)}} \right]_{\pm 1}+\left[ \ln T_{3,1}^{(0)} \right]_{\pm 1} ,
\end{equation}
\begin{equation}
\left[ \ln T_{3,1}^{(0)} \right]_{\pm 1}=-\ln Y_{1,1}^{(0)}Y_{2,2}^{(0)}=- \ln \frac{Y_{-}^{(0)}}{Y_{+}^{(0)}}.
\end{equation}

In the derivation of the excited state TBA equations we can avoid the technical problems coming 
from dealing with branch cuts of the $\log$ functions if we first derive equations 
for the derivatives of the $\log Y$-functions. 
To this end we use the logarithmic derivative of the Y-system (\ref{Y}), 
and the derivative of the discontinuity relations (\ref{Y1cut}-\ref{Yvw1cut}), (\ref{Deltacut0})
and (\ref{Y-cut0}).
Qualitative information about the local singularities of the Y-functions can be read off from
their asymptotic form. Finally we integrate the equations for the derivatives. 
%using the lemma in Appendix E.

In order to be able to extract the necessary analyticity information on the local singularities
of the Y-functions we will make use of the assumption that the exact Y-functions are smooth deformations
of the asymptotic ones. This however cannot be satisfied in the whole complex plane, but only in certain strips (similarity regions). 
We will show that analyticity information regarding the behaviour of our functions in these strips are enough to derive the TBA equations 
and to determine the exact Y-functions.

The Y-functions are smooth deformations of their asymptotic counterparts as long as the $Y_Q^{(0)}$
functions are small. From (\ref{Ya00}) it follows that this condition is satisfied in the region 
${{\Omega}}_{\varepsilon_Q}=\{u \in \mathbb{C}: \quad | \mbox{Im} \, u|<Q/g, \quad |u-u_j^{[\pm(Q-1)]}|> 
\varepsilon_Q \}$,
where $\varepsilon_Q$ is a small but not infinitesimal positive parameter for $Q\geq 2$ and zero
for $Q=1$.
Then the Y-system equations (\ref{Y}) imply for the other Y-functions 
the following similarity regions: 
\begin{itemize}
\item  $Y_Q(u) \sim Y_{Q}^{(0)}(u)=Y_{Q,0}^{(0)}(u) \qquad \, u \in \Omega_{\varepsilon_Q}, \qquad Q=1,2,...,$
\item $Y_{m|vw}^{(\alpha)}(u) \sim  Y_{m|vw}^{(\alpha)(0)}(u)=1/Y_{m+1,\alpha 1}^{(0)}(u)
\qquad |\mbox{Im} \, u|<m/g, \qquad m=1,2,...,$
\item $Y_{m|w}^{(\alpha)}(u) \sim  Y_{m|w}^{(\alpha)(0)}(u)=Y_{1,\alpha(m+1)}^{(0)}(u)
\qquad |\mbox{Im} \, u|<m/g, \qquad m=1,2,...,$
\item $Y_{-}^{(\alpha)}(u) \sim  Y_{-}^{(\alpha)(0)}(u)=-1/Y_{1,\alpha 1}^{(0)}(u), \qquad
|\mbox{Im} \, u|<2/g, \qquad \alpha=\pm,$
\item $Y_{+}^{(\alpha)}(u) \sim  Y_{+}^{(\alpha)(0)}(u)=-Y_{2,\alpha 2}^{(0)}(u), \qquad
|\mbox{Im} \, u|<2/g, \qquad \alpha=\pm.$
\end{itemize}

The discontinuity relations (\ref{Y1cut}-\ref{Yvw1cut}) simplify drastically in the language
of T-functions. The complicated products of Y-functions in the argument of the $\log$ function
become a product of a few T-functions only. In section 4 we will show
that there is a particular choice for the gauge where the exact T-functions are smooth deformations
of the asymptotic ones and due to their simple square-root branch cut structure the right hand sides of
(\ref{Y1cut}-\ref{Yvw1cut}) simplify drastically.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\begin{center}
\psfig{figure=./Yads.eps,width=10cm}
\end{center}
\vspace{-0.5cm}
\caption{\footnotesize
The ${\rm AdS}_5{\rm /CFT}_4$ Y-system. Full circles on the $a$ axis correspond to
massive nodes with $s=0$. The $s$ axis corresponds to nodes with $a=1$.
}
\label{Yads}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\begin{center}
\psfig{figure=./Tads.eps,width=10cm}
\end{center}
\vspace{-0.5cm}
\caption{\footnotesize
The ${\rm AdS}_5{\rm /CFT}_4$ T-system.
The $s$ axis corresponds to nodes with $a=0$.
}
\label{Tads}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



